Explain and Predict, and then Predict Again

A desirable property of learning systems is to be both effective and interpretable. Towards this goal, recent models have been proposed that first generate an extractive explanation from the input text and then generate a prediction on just the explanation called explain-then-predict models. These models primarily consider the task input as a supervision signal in learning an extractive explanation and do not effectively integrate rationales data as an additional inductive bias to improve task performance. We propose a novel yet simple approach ExPred, that uses multi-task learning in the explanation generation phase effectively trading-off explanation and prediction losses. And then we use another prediction network on just the extracted explanations for optimizing the task performance. We conduct an extensive evaluation of our approach on three diverse language datasets -- fact verification, sentiment classification, and QA -- and find that we substantially outperform existing approaches.

==> intro-avi.tex <==
\section{Introduction}
\label{sec:intro}

% The goal of interpretability in learning systems is to describe the internals of a system that explains the decision of a learning system in a way that is understandable to humans. 
% A desirable property of learning systems is to be both effective and interpretable. 
% However, classical models tend to exhibit a natural trade-off between task performance and being interpretable. 
% This has resulted in recently popular post-hoc interpretability approaches that do not negotiate task performance and instead rely on interpreting already trained models in a post-hoc manner.
% However, a key limitation of such post-hoc approaches is that -- explanations might be faithful to the predictions of the model but might not be faithful to the actual decision making process of the model~\citet{rudin2019stop} or to human reasoning~\citet{dissonance19:anand}.
% Secondly, and more worrisome is the problem of evaluation of interpretability techniques due to difficulty in gathering ground truth for evaluating an explanation.
% Methods resorting to human evaluation and simulability are influenced by human-bias~\citet{lage2019evaluation}.
% In this paper, we alternately focus on designing models for language tasks that are interpretable by design and yet deliver promising task performance.


The goal of interpretability in learning systems is to describe the internals of a system that explains the decision of a learning system in a way that is understandable to humans. 
However, classical models are known to exhibit a natural trade-off between task performance and being interpretable.
In this paper, we alternately focus on designing models for language tasks that are interpretable by design and yet deliver promising task performance by exploiting rationales data collected from humans.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/anecdotal.pdf}
    % \vspace{-5mm}
    \caption{\small{ An anecdotal example of output of our \approach{} model that refutes the query using a passage from the \fever{} dataset. The explanation is highlighted in green.}}
    \vspace{-3mm}
    \label{fig:anecdotal_example}
    %\vspace{-3mm}
\end{figure}{}


% A recent paradigm of ensuring interpretability by design is to first generate an extractive explanation given an input, and then consequently use only the explanation for the actual prediction task~\citet{yoon2018:invase,lei2016rationalizing,lehman2019inferring}. \todo{Is Lehman that type of model.}
% An example explanation is shown in Figure~\ref{fig:anecdotal_example}.
% This is attractive because unlike the post-hoc approaches, in such a \emph{explain then predict} one can unambiguosly attribute the reason behind a prediction to the generated explanation.
% One approach to learn an explanations is to additionally collect reasons given by humans, called human rationales, for the prediction task in question.
% These rationales are then utilized as training data for explanation generation~\citet{lei2016rationalizing,deyoung2019eraser}.
% Firstly, approaches like~\citet{lehman2019inferring,yoon2018:invase} cannot \todo{bold claim.did not is fine.} integrate human rationales and are based on optimizing only the final task objective.
% On the other hand, the explanations produced by~\citet{lei2016rationalizing} is not explicitly guided by the training objective.
% Consequently, these approaches although interpretable by design, are not able to considerably improve the task performance. 
% Other modifications to~\citet{lei2016rationalizing} by ~\citet{deyoung2019eraser} using re-inforcement learning for end-to-end training suffers for \todo{I guess suffers from} occasional training degeneration.

A rationale is defined to be a short yet sufficient part of the input text; short so that it makes clear what is most important, and sufficient so that a correct prediction can be made from the rationale alone~\cite{bastings2019interpretable}.  We focus on the explain-then-predict framework that was first proposed by~\cite{lei2016rationalizing} where task prediction is performed in a two-stage manner. In the explanation phase a model learns to extract the rationale from the input text. In the subsequent prediction phase, another independent model predicts the task out solely based on the extractive explanation. 
Unlike the post-hoc approaches the explain-then-predict setup unambiguously attributes the reason for a given prediction to the extractive explanations. However, the challenge for such models has been to attain superior task performance conditioned on the explanation sampled in the explanation phase. 
Approaches that employ this framework typically train in an end to end fashion relying solely on task labels where they negotiate the intractable sampling step by proposing optimization procedures based on REINFORCE~\cite{lei2016rationalizing}, re-parameterization techniques~\cite{bastings2019interpretable} or actor critic approaches~\cite{yoon2018:invase}.  
However these approaches sensitive to hyperparameters can exhibit high variance~\cite{jain2020learning}. 

An alternate way to supervise the explain phase models is to exploit rationales (marked by humans) data~\cite{deyoung2019eraser}. Rationales data has been shown to improve performance of prediction tasks in the past~\cite{zaidan2008modeling,zhang2016rationale,ross:17:right} but these models do not generate explanations.
On the other hand, explain-then-predict models that  do use rationale data train explanation models do not consider the supervision signal from the task in generating explanations~\cite{deyoung2019eraser}. 
Consequently, the generated explanations are not \emph{task-aware} and do not consistently improve task performance (as we show in our experiments).
The main objective of this paper is to exploit supervision signals from both rationales data and task objective for generating \emph{task aware} explanations in order to improve task performance.

% In this paper, we propose a novel yet simple architecture using multi-task learning for the explanation phase where \emph{task prediction} and \emph{explanation generation} are both learned on a common encoder substrate (cf. Figure 2). 
% The common representation learned in the encoder is then used as input in the task specific decoders (either explanation generation or prediction task).
% Using a shared representation space for both prediction and explanation generation provides us the advantage of regularizing the parameters of the common representation substrate using signals from the explanation objective and additionally providing task specific explanations.
% In the prediction phase, the extracted explanation from the explanation is then used to make a final prediction using a model that optimizes explicitly for the task objective. \todo{explanation from the explanation --- is not clear.}

% Since the notion of a rationale may be ambiguous in some contexts and the task of selecting rationales may be challenging to evaluate, we choose to evaluate our methods on three different language tasks where explanations are arguably less ambiguous -- \emph{sentiment classification, question answering} and \emph{fact extraction}.
% We show our MTL framework is able to effectively balance the task and explanation performance by learning to generate task specific explanations.
% More strikingly, we show large improvements (upto $20\%$) in task performance over baselines that are purely optimized for task performance, showing that it is indeed possible to build models that are interpretable by design with the assistance of small amount of rationale data.

Different from earlier approaches, our idea is simple -- since the extractive explanations should be both predictive and explanatory, we aim to learn a better representation of the input using the same set of encoder parameters. 
In our explanation phase of our approach, referred to as \approach, we use multi-task learning where \emph{task prediction} and \emph{explanation generation} are both learned on a common encoder substrate (cf. Figure 2). 
The distinct advantage of such a scheme is that the encoder that is used for explanation gets supervised also from the task-specific signals. 
After the explanation model is trained; in the prediction phase, a separately parameterized model for task prediction is learnt just on the generated explanation. 


We conduct extensive evaluation of \approach{} on three different language tasks where human rationales are provided -- \emph{sentiment classification, question answering} and \emph{fact extraction}.
We find that using a shared representation space for encoding the input for prediction and explanation generation results in more task-specific explanations.  
We also observe that \approach{} is able to effectively balance the task and explanation performance by learning to generate task specific explanations.
More strikingly, our explanations shows large improvements (upto $20\%$) in task performance over baselines that consider full sentences as well as other explain-then-predict competitors. 


==> mtl-fig.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,525); %set diagram left start at 0, and has height of 525

%Flowchart: Prodefined Process [id:dp6715393139116721] 
\draw  [fill={rgb, 255:red, 246; green, 246; blue, 245 }  ,fill opacity=1 ] (181.4,310.8) -- (241.4,310.8) -- (241.4,380.8) -- (181.4,380.8) -- cycle ; \draw   (188.9,310.8) -- (188.9,380.8) ; \draw   (233.9,310.8) -- (233.9,380.8) ;
%Shape: Square [id:dp44037023084927873] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 213 }  ,fill opacity=1 ] (383,310.4) -- (452,310.4) -- (452,379.4) -- (383,379.4) -- cycle ;
%Curve Lines [id:da17463850597309416] 
\draw [color={rgb, 255:red, 169; green, 43; blue, 43 }  ,draw opacity=0.83 ]   (241,352) .. controls (280.4,322.45) and (329.5,369.84) .. (379.71,345.18) ;
\draw [shift={(382,344)}, rotate = 511.84] [fill={rgb, 255:red, 169; green, 43; blue, 43 }  ,fill opacity=0.83 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da955781061506505] 
\draw    (452.4,348.9) -- (499.4,349.19) ;
\draw [shift={(501.4,349.2)}, rotate = 180.35] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (195.2,336.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {MTL};
% Text Node
\draw (273.2,317) node [anchor=north west][inner sep=0.75pt]   [align=left] {Explanation};
% Text Node
\draw (136.8,385.4) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont The movie \textbf{\textcolor[rgb]{0.72,0.11,0.11}{was aweful}} }\\{\fontfamily{pcr}\selectfont in the second half}};
% Text Node
\draw (353.6,384.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont ... was aweful ...}};
% Text Node
\draw (462,325.4) node [anchor=north west][inner sep=0.75pt]   [align=left] {Task Prediction};
% Text Node
\draw (408,278.2) node [anchor=north west][inner sep=0.75pt]    {$f\prime $};
% Text Node
\draw (149.2,277.4) node [anchor=north west][inner sep=0.75pt]    {$f^{T}_{ \begin{array}{l}
\{\theta ,\ \phi _{T}\}\\
\end{array}}$};
% Text Node
\draw (221.6,279.8) node [anchor=north west][inner sep=0.75pt]    {$f^{E}_{ \begin{array}{l}
\{\theta ,\ \phi _{E}\}\\
\end{array}}$};


\end{tikzpicture}


==> old-span-based.tex <==
\subsection{Span-based Rationale Prediction}
Like earlier, we use \bert{} as the shared encoder for both the task and explanation.

% \textbf{Task prediction:} The task classification framework is kept same as \methodindv. The CLS token is passed through the MLP layer to predict the task output. 

\textbf{Explanation prediction.} The explanation part is different from \methodindv. Rather than classifying each token separately, we follow the \textit{pointer network} approach proposed by Vinyals~et~al.~\cite{vinyals2015pointer} to predict rationales as intervals over token sequence by their start and end positions. In following descriptions, $|S|$ is the length of the whole sequence, and the dimension of representation of each token is $d_{rep}$ (i.e., the representation matrix $M_S$ of the passage $S$ is $|S|\times d_{rep}$); $\mbox{\bilstm}$ denotes a bidirectional LSTM~\cite{schuster1997bidirectional, hochreiter1997long} layer and $M^i$ represents the $i$-th row of matrix $M$. Specifically, if $M$ is the representation matrix, $M^i$ is the embedding vector corresponding to the $i$-th token. The structure of the explanation part is as follows: 
    
  
First, the sub-token embeddings of the representation model are passed to a \bilstm.

\begin{equation}
    \label{eq:first_rnn}
    M_1 = \mathtt{Bi-LSTM}\left(M_S\right)\mbox{,}
\end{equation}
    where $M_1$ is a $|S|\times 2d$ matrix, $d$ is the output dimension of a LSTM unit.
    Then the following MLP layer predicts the possibility of each token $x^i$ at position $i$ being the start token:
    \begin{equation}
    \label{eq:p_start}
    p(x_{start}^i) = \sigma\left(\mathbf{W}_1M_1^T\right)\mbox{,}
    \end{equation}
    where $\mathbf{W}_1$ is the matrix with trainable parameters of shape $|S|\times 2d$, $\sigma$ is the element-wise sigmoid function. 
    
    After predicting the start points, we weight $M_1$ by the probability of these start points, then sum the weighted matrix across the whole sequence of tokens. The result vector is again element-wise multiplied with the representation of each sub-token:
    \begin{equation}
        \label{eq:start_attention}
        \tilde{M}_1^i = M_1^i \odot \sum_{j=1}^{|S|}p(x_{start}^j)M_1^j\mbox{,}
    \end{equation}{}
    where $\odot$ is element-wise (Hadamard) product and $p(x_{start})$-s here serve like attention weights.
    The second \bilstm{} takes concatenated $M_S$, $M_1$, $\tilde{M}_1$ and $M_1\odot \tilde{M}_1$ as input:
    \begin{equation}
        \label{eq:second_rnn}
        M_2 = \mathtt{BiLSTM}\left( [M_S; M_1, \tilde{M}_1, M_1 \odot \tilde{M}_1] \right)\mbox{,}
    \end{equation}{}
    where the input matrix is in shape of $T\times (d_{rep} + 6d)$ and the shape of $M_2$ is $T\times 2d$.
    
    Finally we calculate the possibility of each token $y^j$ at position $j$ being the end point given each previous token being the start point, i.e.
    \begin{align}
        p(y_{end}|x_{start}) = \mathtt{Softmax}\left(U\odot\mathbf{W}_2[M_S;M_2]^T\right)
    \end{align}
    
    where $U$ is the upper-triangular matrix of size $L\times L$, since we are only interested of end tokens locating after corresponding start tokens; $\mathbf{W}_2$ is an $L \times (d_{rep}+2d)$ dimensional trainable matrix. Figure~\ref{fig:mtl-pointer-example} shows the diagram of this approach.
    
    %\todo{Done upto this point}
    

\textbf{Loss function:} We sum up the classification and explanation loss together int he same manner as in the method 1~(Eqn.~\ref{eqn:loss_function}), where the loss function for the classification task even remains the same ($\mathcal{L}_{cls}$). However, the explanation loss ($\mathcal{L}_{exp}$) in this method is modeled in a different way. It consists of two parts, i.e., concordance of start position of each evidence and concordance of end positions given the starts. These two components are modeled separately. First, we predict the possibility of each individual token to be a start token for a rationale interval and the loss function is the sum of binary cross entropy over all the tokens.
\begin{equation}
        \mathcal{L}_{start} = \sum_{i=1}^{|S|}(1-t^i)(1-p(x_{start}^i)) + t^ip(x_{start}^i)\mbox{,}
\end{equation}
where $t^i$ is $1$ when the $i$-th token is a start token of an rationale interval.
Next, the loss function of the end points is calculated by summing up the log-inverse $p(y^j_{end}|x^i_{start})$ for all evidence intervals, where the $i$-th token is a start token and the $j$-th token is the end token of the corresponding evidence interval.
    
\begin{equation}
        \mathcal{L}_{end} = \sum_{e\in E}\log \frac{1}{p\left(e_{end}|e_{start}\right)}\mbox{,}
\end{equation}
    
where $E$ is the set of evidence intervals, $e_{start}$  and $e_{end}$ indicates the start and the end token of this interval.
Finally, the explanation loss is the sum of two parts, i.e.
    \begin{equation}
        \mathcal{L}_{exp} = \mathcal{L}_{start} + \mathcal{L}_{end}
    \end{equation}
    

==> table-anecdotal.tex <==
\begin{table*}[tbh]
\centering
\caption{Example rankings with axiomatic explanations: Document IDs from Robust04 have a suffix~$+$~($-$) for (non-)relevant TREC judgments. Axiomatic explanations show how many axioms would rank this search result the same as ($\Leftrightarrow$), higher than ($\uparrow$) or lower than ($\downarrow$) the retrieval system, followed by up to three most relevant axioms, annotated with how many other results they rank the same (superscript) or differently (subscript) relative to this document.
}
\label{table-ranking-examples}
\footnotesize
\providecommand{\AXSP}[3]{\ensuremath{%
\mathrm{#1}^{\textcolor{green!40!black}{#2}}_{\textcolor{red!75!black}{#3}}%
}}
\begin{tabular}{@{}rl@{~}lll@{}}
\toprule
    \multicolumn{3}{@{}l@{}}{
    {\bfseries System:}~DRMM
    \qquad
    {\bfseries Query:}~367
    \quad
    ``piracy''
    }
    &
   \multicolumn{2}{l@{}}{\bfseries Axiomatic explanation} 
    \\[.5ex]
\multicolumn{2}{@{}l}{\bfseries Rank Docid}&
\bfseries Content &
\bfseries \tiny $ \Leftrightarrow/~\uparrow/~\downarrow $ &
\bfseries Most relevant axioms \\
\midrule
 1 &  FT944-16684$^{-}$ &  Software companies offer rewards in anti-piracy drive -- Leading software compan\dots &  1 / 0 / 1 &  $\AXSP{REG}{9}{0}$\quad $\AXSP{DIV}{3}{6}$ \\
 2 &  FT931-8281$^{-}$ &  Survey of personal and portable computers (21): tougher times for pirates / a lo\dots &  2 / 0 / 1 &  $\AXSP{REG}{8}{1}$\quad $\AXSP{DIV}{4}{5}$\quad $\AXSP{LNC1}{1}{0}$ \\
 3 &  FT934-14966$^{-}$ &  Sixties buccaneer deals in high-tech piracy -- In his days as a radio caroline p\dots &  3 / 0 / 3 &  $\AXSP{DIV}{4}{5}$\quad $\AXSP{REG}{3}{5}$\quad $\AXSP{STMC2}{1}{0}$ \\
 4 &  FT911-1567$^{-}$ &  A rich haul from the sound of music: the illicit copying and sale of recorded mu\dots &  3 / 1 / 0 &  $\AXSP{REG}{7}{2}$\quad $\AXSP{DIV}{4}{5}$\quad $\AXSP{LNC1}{1}{0}$ \\
 5 &  LA032889-0045$^{-}$ &  Busting cable pirates; simi valley piracy case is one of the first to result in \dots &  3 / 1 / 0 &  $\AXSP{REG}{6}{1}$\quad $\AXSP{DIV}{4}{5}$\quad $\AXSP{LNC1}{2}{0}$ \\
 6 &  FBIS3-43017$^{-}$ &  Computer piracy in russia is a widespread phenomenon. the world average ratio of\dots &  5 / 1 / 0 &  $\AXSP{REG}{6}{1}$\quad $\AXSP{DIV}{3}{5}$\quad $\AXSP{LNC1}{1}{0}$ \\
 7 &  FBIS3-42979$^{-}$ &  Computer piracy in russia is a widespread phenomenon. the world average ratio of\dots &  2 / 1 / 0 &  $\AXSP{REG}{6}{1}$\quad $\AXSP{DIV}{3}{5}$\quad $\AXSP{LNC1}{1}{0}$ \\
 8 &  FT923-9880$^{+}$ &  Jakarta sinks plan to combat piracy -- Plans for an international centre to figh\dots &  5 / 0 / 0 &  $\AXSP{REG}{8}{1}$\quad $\AXSP{DIV}{8}{1}$\quad $\AXSP{STMC2}{2}{0}$ \\
 9 &  FT944-9277$^{-}$ &  Uk company news: bskyb says piracy could undermine float confidence -- British s\dots &  2 / 1 / 0 &  $\AXSP{DIV}{8}{1}$\quad $\AXSP{REG}{8}{0}$\quad $\AXSP{LNC1}{0}{1}$ \\
 10 &  FT924-15875$^{-}$ &  Piracy warnings -- A 24-hour centre to counter piracy in the seas of south-east \dots &  2 / 0 / 0 &  $\AXSP{DIV}{9}{0}$\quad $\AXSP{REG}{9}{0}$
  \\[1ex]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ranking 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\toprule
    \multicolumn{3}{@{}l@{}}{
    {\bfseries System:}~DRMM
    \qquad
    {\bfseries Query:}~425
    \quad
    ``counterfeiting money''
    } &
\bfseries \tiny $ \Leftrightarrow/~\uparrow/~\downarrow $ &
\bfseries Most relevant axioms \\
\midrule
 1 &  FBIS3-58171$^{+}$ &  The head of the gang that wanted to circulate some 970,000 counterfeit dollars i\dots &  6 / 0 / 5 &  $\AXSP{PROX5}{8}{1}$\quad $\AXSP{PROX3}{7}{2}$\quad $\AXSP{STMC1\_f}{7}{2}$ \\
 2 &  FBIS4-46741$^{+}$ &  Crime counterfeiting is probably one of the world's oldest and most widespread t\dots &  10 / 0 / 1 &  $\AXSP{PROX2}{7}{2}$\quad $\AXSP{PROX3}{7}{2}$\quad $\AXSP{REG}{7}{2}$ \\
 3 &  FBIS4-26260$^{+}$ &  The hongqiao district people's court examined and concluded a case of traffickin\dots &  5 / 0 / 5 &  $\AXSP{PROX4}{7}{2}$\quad $\AXSP{PROX5}{7}{2}$\quad $\AXSP{PROX2}{7}{2}$ \\
 4 &  LA091590-0091$^{+}$ &  Plumbers discover cash flow problem in sewer; counterfeiting: phony \$100 bills a\dots &  7 / 2 / 0 &  $\AXSP{PROX4}{7}{2}$\quad $\AXSP{PROX5}{7}{2}$\quad $\AXSP{PROX1}{6}{3}$ \\
 5 &  FBIS3-54773$^{+}$ &  On 25 december a criminal gang of six chechnya inhabitants was arrested in st. p\dots &  7 / 1 / 2 &  $\AXSP{PROX4}{7}{2}$\quad $\AXSP{PROX5}{7}{2}$\quad $\AXSP{REG}{5}{4}$ \\
 6 &  LA102189-0077$^{+}$ &  California in brief; modesto; man indicted in counterfeiting -- A federal grand \dots &  7 / 3 / 0 &  $\AXSP{PROX4}{7}{1}$\quad $\AXSP{PROX5}{6}{3}$\quad $\AXSP{PROX1}{6}{3}$ \\
 7 &  FBIS4-47199$^{+}$ &  The number of counterfeit ruble bank notes, bank notes of convertible currency, \dots &  7 / 4 / 0 &  $\AXSP{PROX5}{8}{1}$\quad $\AXSP{STMC1}{6}{3}$\quad $\AXSP{PROX4}{6}{1}$ \\
 8 &  FBIS4-58263$^{+}$ &  Counterfeit, 1990-issue  \$100 bills have recently found their way onto the jorda\dots &  6 / 4 / 0 &  $\AXSP{PROX4}{7}{2}$\quad $\AXSP{REG}{7}{2}$\quad $\AXSP{PROX3}{7}{1}$ \\
 9 &  FBIS4-59139$^{+}$ &  For some time, tel aviv has anxiously been raising with egyptian politicians an \dots &  10 / 1 / 0 &  $\AXSP{PROX1}{8}{1}$\quad $\AXSP{PROX3}{8}{1}$\quad $\AXSP{PROX2}{8}{1}$ \\
 10 &  LA010390-0055$^{-}$ &  Rival athletic shoe makers formed an alliance to battle counterfeits -- When u.s\dots &  6 / 5 / 0 &  $\AXSP{PROX1}{9}{0}$\quad $\AXSP{PROX4}{8}{1}$\quad $\AXSP{PROX5}{8}{1}$ \\
\bottomrule

\end{tabular}
\end{table*}
 

==> trash bin/01.intro.tex <==
\section{Introduction}
\label{sec:intro}

The goal of interpretability is to describe the internals of a system that explains the decision of a learning system in a way that is understandable to humans. 
This is necessary to be able to verify and understand the underlying basis for the decisions. 
Most of the popular post-hoc approaches are based on optimising \emph{fidelity}, i.e., the ability of being faithful or similar to the predictions of an already trained black-box model.
This is operationalized by approaches that (a) only operate on the parameters of an already-trained machine learning model~\citet{montavon-pr17} and (b) focus on generating a proxy model that approximates the decisions of the original black box model~\citet{ribeiro2016should:lime}.
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/anecdotal_evidences/anecdotal.pdf}
    \vspace{-5mm}
    \caption{{\bf An anecdotal example of output of our MTL model that refutes the query using a passage from the \fever{} dataset. The explanation is highlighted in gray.}}
    \vspace{-3mm}
    \label{fig:anecdotal_example}
    %\vspace{-3mm}
\end{figure*}{}

The key limitation in using fidelity as a measure of accuracy of interpretability is that -- explanations might be faithful to the predictions of the model but might not be faithful to the actual decision making process of the model~\citet{rudin2019stop} or to human reasoning~\citet{dissonance19:anand}.
Secondly, and more worrisome is the problem of evaluation of interpretability techniques due to difficulty in gathering ground truth for evaluating an explanation.
Methods resorting to human evaluation and simulability are influenced by human-bias~\citet{lage2019evaluation}.

We follow an alternate design principle that is to gather human explanations or rationales~\citet{zaidan2008modeling,lei2016rationalizing} for training instances prior to model training.
We then train the model for optimising the task objective while taking into account the human rationale for a prediction.
A distinct advantage of such an approach is that the trained model enforces human interpretability during training ensuring the model is right for the right reasons.
There have been previous attempts that utilize training with rationales~\citet{zaidan2007using,lei2016rationalizing,ross:17:right} but they suffer from some key limitations.
In~\citet{zaidan2008modeling, ross:17:right} rationales are only used for improving task performance by designing regularizers that utilize rationales.
~\citet{lehman2019inferring,lei2016rationalizing} explicitly generate extractive explanations by using a staged architecture where explanations are generated first, called hard selection. 
~\citet{deyoung2019eraser} tries to propose comprehensive explanations by considering all possible extracted explanations in a soft selection approach.
However, both these staged approaches affect task performance due to inherent information loss in the first explanation stage.

In this paper, we propose a novel yet simple architecture using a multi-task learning where \emph{task prediction} and \emph{explanation generation} are both learned on a common encoder substrate (cf. Figure 2). 
The common representation learned in the encoder is then used as input in the task specific decoders (either explanation generation or prediction task).
Using a shared representation space for both prediction and explanation generation provides us the advantage of regularizing the parameters of the common representation substrate using signals from the explanation objective.
We propose to train the model in a multi-task learning setting with different learning objectives for the explanations -- based on \emph{spans} and \emph{independent extractive tokens}.



Since the notion of a rationale may be ambiguous in some contexts and the task of selecting rationales may be challenging to evaluate, we choose to evaluate our methods on three different language tasks where explanations are arguably less ambiguous -- \emph{sentiment classification, question answering} and \emph{fact extraction}.
We show our MTL framework is able to effectively balance the task and explanation performance.
More strikingly, we show up to $2.5$x improvement in explanation performance (measured by AUPRC) compared to soft-selection methods.
An example explanation is shown in Figure~\ref{fig:anecdotal_example}.
% To have a quick first glance at to which extent our proposal approaches, here we show a model's output by an anecdotal example \ref{fig:anecdotal_example}. This example involves a crop of an instance from the \fever{} dataset. The model predicts whether the query is \textbf{SUPPORT}ed or \textbf{REFUTE}d by the passage, in the same time marking the rationale supporting the classification from the passage.


==> trash bin/02.relwork.tex <==
\section{Related Work}
\label{sec:rel-work}

% \textbf{what is a rough classification of interpretability approaches ?}

The classical approach in machine learning to enforce interpretability while learning from data is to constrain the choice of models to those that are \emph{interpretable by design}.
This can either be realized through regularization techniques such as Lasso that attempts to choose a small subset of the most important features, or by using models that structurally match human reasoning such as Bayesian Rule Lists~\citet{letham2015interpretable}, Supersparse Linear Integer Models~\citet{ustun2016supersparse}, or Probabilistic Scaling~\citet{choudhury1997probabilistic}. 

\textbf{Post-hoc interpretability.} 
Unlike ensuring interpretability by design, a majority of the recent approaches focuses on post-hoc explanations where the task of interpretability is to explain the decisions of an already trained model post training.
Post-hoc models are either \emph{model-agnostic} where the interpretability approach has no access to the trained model parameter.
Different from the model-agnostic approaches, \emph{model introspective approaches} are post-hoc methods that have full access to the parameters of the model to be interpreted and attribute importance to input features~\citet{lundberg2017unified,ribeiro2016should:lime}, parameters~\citet{xu2015show} or data~\citet{koh2017understanding}.

% \textbf{Interpretability by analyzing attention.}

An alternate line of work that performs post-hoc analysis of already learnt neural models by analyzing state activation~\citet{NIPS2013_5166, karpathy2015visualizing}~\citet{li2016understanding} or attention weights~\citet{bahdanau2014neural, cheng2016long, martins2016softmax, cui2016attention, xu2015multi, yang2016hierarchical}.
The attention weights learnt as weights assigned to token representation are intended to describe rationales.
However, recently the faithfulness of interpreting model prediction with soft attention weights has been called into question (\citet{wiegreffe2019attention, jain2019attention}). 
Specifically, contextual entanglement of inputs is non-trivial and the prediction model can still perform well even if the attention weights don't correlated with the (sub-)token weight as desired by human.
Our approach for rationale based explanations differ in the type of architectures, objectives and general nature of its utility. 

% \textbf{How is it different from Rationale based classification.} 

\textbf{Rationale-based interpretability.} The closest to our work is the work on rationale classification and has roots in the seminal work of~\citet{zaidan2008modeling,zaidan2007using} that aims to improve model generalization by utilizing human rationales as inductive bias.
Alternately~\citet{lei2016rationalizing} proposed a sequential approach of rationale generation followed by prediction using the generated prediction.
Specifically, their approach is naturally separated into two components: generator and encoder, where the generator selects short subsets of original text that are sufficient for the encoder to make consistent predictions. 
The model employs reinforcement learning \citet{williams1992simple} to train both components jointly. 
\citet{lehman2019inferring} uses a similar philosophy of decoupling rationale generator and predictor albeit a slightly different architecture. 
Such pipelined approaches that learn a task predicted purely on the predicted explanation tokens are referred to as \emph{hard selection} approaches.
On contrary, \textit{soft-selection} approaches optimize the models only for the task and attention scores are used as a proxy to extract and rank the tokens/phrases as an explanation for the task~\citet{deyoung2019eraser}.


% Furthermore, Yu et al. propose a different approach in \citet{yu2019rethinking}. Rather than explicitly separates the evidences selector (generator) and the classifier (encoder), the generator and the encoder are entangled in their approach. 


All these approaches suffer from two critical deficiencies. Firstly, with a strong separation of parameters in the pipelined approaches do not use the same parameters for prediction and explanation. 
Moreover, since the rationale explanation is precursor to the prediction phase results in information loss resulting in the final accuracy of the classification task.
We focus on generation of rationales using the same parameter space used for predictions using a multi-task learning framework.




==> trash bin/05.experiments.backup.tex <==
%\newpage
\section{Experimental Evaluation}
\label{sec:eval}
Our primary research questions that we experimentally evaluate are:

% \noindent \textbf{1.}~How effective is the Multi-Task Learning (MTL) framework for joint task and explanation learning? \\
% \noindent \textbf{2.}~What is task-explanation accuracy trade-off in MTL framework? \\
% \noindent \textbf{3.}~What impact does $\lambda$ have on task and explanation accuracy? 
\begin{enumerate}
    \item [\textbf{RQ 1}] How effective is the Multi-Task Learning (MTL) framework for joint task and explanation learning?
    \item [\textbf{RQ 2}] What are the task-explanation performance trade-offs in an MTL framework?
    
    \item[\textbf{RQ 3}] What impact does $\lambda$ have on task and explanation performance ? 
\end{enumerate}

We first describe the baselines, experimental setup, and dataset details. In the next section, we elaborate on the experimental results in details.

\subsection{Training setup and Hyper-parameters}
\label{sec:parameter_setup}
We consider \bertbase{} as the shared encoder model with $\textrm{MAX\_SEQ\_LEN}=512$ and the warm-up proportion $0.1$. Both the models are trained using Adam optimizer~\citet{kingma2014adam} with a batch size of 16, and $\textrm{learning\_rate}=1e-5$. Models are trained for 10 epochs with early-stopping criteria on the validation set and $\textrm{patience}=3$.

The MLP for the task classification consists of a $256$ dimensional hidden dense layer followed by an Sigmoid output layer. The explanation part of \methodindv{} consists of a 128-dimensional GRU with uniform random kernel analyzer. \methodspan{} contains two \bilstm{} networks of 100 dimensions (i.e., $d=100$). The final outputs of the explanation part correspond to the sub-token representations of~\bert. Hence, some adjacent sub-tokens are merged to their corresponding original words and their explanation are also combined using max-pooling.

% The optimum $\lambda$s are selected based on the performance on validation set by sweeping over a range of $[0.1,500]$ (\methodindv{}) or $[0.001, 5]$ (\methodspan{}). For optimal $\lambda$ selection, we consider 10\% and 25\% of the \fever{} and \multirc{} datasets respectively to avoid overfitting issue. The optimal $\lambda$ values are chosen according to the performance on validation set and are noted in Tables~\ref{table:task_explanation_result_hard} and \ref{table:task_explanation_result_soft}. 

\textcolor{red}{Zijian: The optimal $\lambda$-s are separately decided for \mtlsoft and \mtlhard. For \mtlsoft it is decided by model's performance on both the classification task (\textbf{Macro-Avg-F1}) and the concordance of the MR (Machine Rationales, as the distribution over sub-tokens) with the given HA (Human Annotation), namely the \textbf{AUPRC}. The distributions over the sub-tokens from a single original token are max-pooled. While for \mtlhard the best $\lambda$-s are also decided by its performance on both tasks, namely (\textbf{Macro-Avg-F1}) and token-wise F1 (\textbf{Token-F1}) of the MAs. The corresponding optimal $\lambda$-s are noted in the table}

All experiments are conducted on an Nvidia 32GB V100 using Tensorflow~\citet{abadi2016tensorflow} framework.

\noindent\textbf{Baselines:} We consider the following six baselines from the Eraser work~\citet{deyoung2019eraser}: (i).~\textbf{\citet{lei2016rationalizing}:} Hard selection based approach proposed by Lei~et~al. Encoder is trained with annotated rationales and decoder has to predict the task based on extracted rationales, (ii). ~\textbf{\citet{lei2016rationalizing}(u):} Similar to first baseline but rationale level supervision is missing. Model learns directly from task level supervision using Reinforce estimator loss, (iii).~\textbf{\citet{lehman2019inferring}:} It is a pipeline approach where first model is trained to identify the rationales and the next one is trained on those rationales to predict the task, (iv).~\textbf{Bert-To-Bert:} Similar to the model proposed by Lehman~et~al~\citet{lehman2019inferring} but BERT is used as encoder and decoder instead of LSTM. (v)~\textbf{BERT-LSTM + Attention:} This has only task-level supervision and rationales are extracted based on attention score. Glove embeddings are considered for \fever{} instead of \bert{} due to computational constraint, (vi).~~\textbf{BERT-LSTM + Simple Gradient:} Same as (v) but tokens are ranked based on gradients.

\subsection{Metrics} 

We consider six different metrics considered in earlier work~\citet{lei2016rationalizing,deyoung2019eraser}.

\textbf{F1 Measures.} We consider two F1 measures, \textbf{Macro F1} for the classification task and ~\textbf{token F1} for the rationale task.

\textbf{AUPRC.} or area under the precision-recall curve since for soft-annotation for each token is assigned with a ranking score (sometimes probability of being rationale).

\textbf{IOU (Intersection-Over-Union) F1.} considers a prediction as true positive if its token-wise IOU (length of overlap divided by length of union) is larger than a threshold (we choose the threshold to be $0.5$ to be consistent with the measurements in prior works).

\textbf{Comprehensiveness and Sufficiency.}
Proposed by~\citet{deyoung2019eraser} the~\textbf{comprehensiveness} of a rationale $r_{ij}$ on instance $i$ and class $j$ is defined as $\mbox{comprehensiveness}(r)=\hat{p}_{ij}-\tilde{p}_{ij}$, where $\hat{p}_{ij}$ is model's prediction on the original input, and $\tilde{p}_{ij}$ is prediction over the input where the rationale $r_{ij}$ is stripped. 
~\textbf{Sufficiency} on the other hand is defined as the complement of the comprehensiveness, $\mbox{sufficiency}=\hat{p}_{ij}-\bar{p}_{ij}$, where $\bar{p}_{ij}$ is the predicted probability using \emph{only} rationale $r_{ij}$;



The first metric is for the task accuracy measurement and rest of the metrics are related to the quality of rationale generation.

\subsection{Datasets}

We consider three diverse language tasks for our evaluation.

\textbf{\movie}~\citet{zaidan2007using,zaidan2008modeling}. One of the original datasets providing extractive rationales, the movies dataset has \textit{pos}itive or \textit{neg}ative sentiment labels on movie reviews. As the included rationale annotations are not necessarily comprehensive (i.e., annotators were not asked to mark \emph{all} text supporting a label), we collect a comprehensive evaluation set on the final fold of the original dataset~\citet{pang2004sentimental}

\textbf{ \fever}~\citet{Thorne18Fever} (short
for Fact Extraction and VERification) is a fact-checking dataset. 
The task is to verify claims from textual sources. 
In particular, each claim is to be classified as \textit{supported}, \textit{refuted} or \textit{not enough information} with reference to a collection of potentially relevant source texts.  
We follow the setup of ~\citet{deyoung2019eraser} who restrict this dataset to \textit{supported} or \textit{refuted}.


\textbf{ \multirc}~\citet{khashabi2018looking}. This is a reading comprehension dataset composed of questions with multiple correct answers that by construction depend on information from multiple sentences. In \multirc{}, each Rationale is associated with a question, while answers are independent of one another. We convert each rationale/question/answer triplet into an instance within our dataset. Each answer
candidate then has a label of \textit{True} or \textit{False}.

% \begin{itemize}
%     \item \movie, first introduced by Zaidan~et~al.~\citet{zaidan2007using, zaidan2008modeling}, was initially meant to fortify training process of sentiment classifiers by providing rationales supporting corresponding sentiment. This dataset is further re-annotated by~\citet{deyoung2019eraser} to make it more comprehensive.
%     \item \fever~\citet{Thorne18Fever}, a large scale Fact Extraction and VERification dataset. 
%     \item \multirc \citet{khashabi2018looking} is a reading comprehension Q-A dataset. Each question may have multiple answers constructed based on multiple sentences of the input document.
% \end{itemize}
The train/val/test set are kept the same as provided ~\citet{deyoung2019eraser}. 

% The other datasets either contain mostly too-long-documents (e.g. \boolq{}~\citet{clark2019boolq} and \evidenceinference{}~\citet{lehman2019inferring}), or is ternary (\esnli{}~\citet{NIPS2018_8163esnli}) even multi-categories classification (\cose{}~\citet{rajani2019explaincose}) datasets.


%In this paper, we mainly focus on the interpretation on sequence classification tasks. This type of task are well researched in recent years and many models with impressive predictive performance have been published. Their application in critical fields, however, such as in  policy-making\citet{brennan2013emergence} or in science \citet{angermueller2016deep} are highly restricted.

% \subsection{Hyper-parameters and implementation details}
% In the experiments we use \bertbase~as our language representation model, the length of input is set to $\textrm{MAX\_SEQ\_LEN}=512$ and the warm-up proportion of \bert~is set to $0.1$. For both approaches the following hyper-parameters are used in common: $\textrm{batchsize}=16$, initial learning rate of Adam \citet{kingma2014adam} is $\textrm{learning\_rate}=1e-5$, $\textrm{train\_epochs}=10$ with early-stop focusing on validation loss with $\textrm{patience}=3$. Model checkpoints performs the best on the evaluation set are kept.

% The MLP for the classification task consists of one hidden Dense layer with $256$ dimensions and an output layer with sigmoid as its activation function.the GRU layer in our \gru{} approach has $128$ dimensions and uniform random kernel initializer. The sequential outputs of the GRU layer are passed to the output layer with sigmoid activation directly. in our \rnr approach, both bidirectional LSTM are $100$ dimensions, i.e. $d=100$. The final outputs of the explanation part correspond to sub-token representations of~\bert. Therefore some adjacent sub-tokens are merged to their corresponding original words, while their explanation are also combined using max-pooling.

% The optimum $\lambda$ used in both approach for three dataset are chosen independently by sweeping through possible values $\lambda$, where $\lambda$ varies in log-scale. Because \fever~and \multirc are seemingly large datasets, only $10\%$ and $25\%$ of the original datasets are used for finding the optimal hyper-parameters. The optimal $\lambda$-s are chosen according to their performance on evaluation set and are noted in table~\ref{table:downstream}.

% Our implementation is based on Tensorflow \citet{abadi2016tensorflow} version 1.14.1 and has been verified useful with version 2.0.0-beta1. The experiments are accomplished on 2xNVIDIA Tesla V100.

% \subsection{Datasets}
% The dataset we choose is a subset of those provided in the interpretability evaluation benchmark ERASER\citet{deyoung2019eraser}. The three datasets we used are as follows:
% \begin{itemize}
%     \item \movie, first provided in \citet{zaidan2007using, zaidan2008modeling}, was initially meant to fortify training process of sentimental classifiers by providing extractive rationals supporting corresponding sentiment. This dataset was latter on modified by \citet{deyoung2019eraser} to make it more comprehensive.
%     \item \fever~\citet{Thorne18Fever}, a large scale Fact Extraction and VERification dataset. 
%     \item \multirc \citet{khashabi2018looking} is a reading comprehension Q-A dataset. To each question there are multiple answer, and these answer are constructed depend on multiple sentence of the input document. 
% \end{itemize}
% The train/val/test set are kept the same as provided in the ERASER \citet{deyoung2019eraser}.



==> trash bin/05.experiments.tex <==
%\newpage
\section{Experimental Evaluation}
\label{sec:eval}
Our primary research questions that we experimentally evaluate are:
% [下午2:21] Avishek Anand
%     so our design space is the following hard selection approaches 1) MTL + TASK, 2) EXP + TASK, 3) Competitors....EXP is when you use BERT only to optimize the explanation task and do not consider the task like in MTL
% 已编辑​[下午2:22] Avishek Anand
%     so RQ1: how does 1) compare vs 2) for Task performance 
% ​[下午2:23] Avishek Anand
%     RQ2: How does explanations from MTL (2) compare against only predicting the explanations (2)

\begin{enumerate}
    \item [\textbf{RQ 1}] What are the task-explanation performance trade-offs in the MTL framework?%deciding the lambdas
    \item [\textbf{RQ 2}] How is the classification task performance of the \mtlhard?
    \item [\textbf{RQ 3}] How is the quality of the explanation from the \mtlhard compared with 1) explanation emitted by the explanation-only model  and 2) explanation annotated by human?
    \item [\textbf{RQ 4}] How is the performance of \mtlsoft compared with other compatitors presented in \citet{deyoung2019eraser}?
\end{enumerate}

We first describe the experimental setup, baselines, and dataset details. In the next section, we elaborate on the experimental results in details.


\subsection{Training setup and Hyper-parameters}
\label{sec:parameter_setup}
We consider \bertbase{} as the shared encoder model with $\textrm{MAX\_SEQ\_LEN}=512$ and the warm-up proportion $0.1$. Both the models are trained using Adam optimizer~\citet{kingma2014adam} with a batch size of 16, and $\textrm{learning\_rate}=1e-5$. Models are trained for 10 epochs with early-stopping criteria on the validation set and $\textrm{patience}=3$.

The MLP for the task classification consists of a $256$ dimensional hidden dense layer followed by an Sigmoid output layer. The explanation part consists of a 128-dimensional GRU with uniform random kernel analyzer. The final outputs of the explanation part correspond to the sub-token representations of~\bert. Hence, some adjacent sub-tokens are merged to their corresponding original words and their explanation are also combined using max-pooling.

\textcolor{red}{Zijian: The optimal $\lambda$-s are separately decided for \mtlsoft and \mtlhard. For \mtlsoft it is decided by model's performance on both the classification task (\textbf{Macro-Avg-F1}) and the concordance of the explanation with the given HA (Human Annotation), namely the \textbf{AUPRC}. While for \mtlhard the best $\lambda$-s are also decided by the performance of both the classifier and the explainer. The matrics used here are namely (\textbf{Macro-Avg-F1}) and token-wise F1 (\textbf{Token-F1}) of the explanations. The corresponding optimal $\lambda$-s are noted in the results table.}

Whenever the ablation of some sub-sequences from the input text is involved in the experiment, we mark them by wild-card tokens\footnote{the periods ('.') are used}. Because the contextual representation models also take token position as a part of input features, e.g. the position encoding in \bert{}, we cannot simply strip such sub-sequences and concatenate their predecessor and successors together.

All experiments are conducted on an Nvidia 32GB V100 using Tensorflow~\citet{abadi2016tensorflow} framework.

\noindent\textbf{Baselines:} We consider the following baselines, six of them are from the Eraser work~\citet{deyoung2019eraser}:
\begin{enumerate}
    \item[i]\textbf{\citet{lei2016rationalizing}:} Hard selection based approach proposed by Lei~et~al. Encoder is trained with annotated rationales and decoder has to predict the task based on extracted rationales;
    \item[ii]\textbf{\citet{lei2016rationalizing}(u):} Similar to first baseline but rationale level supervision is missing. Model learns directly from task level supervision using Reinforce estimator loss;
    \item[iii]\textbf{\citet{lehman2019inferring}:} It is a pipeline approach where first model is trained to identify the rationales and the next one is trained on those rationales to predict the task;
    \item[iv]\textbf{Bert-To-Bert:} Similar to the model proposed by Lehman~et~al~\citet{lehman2019inferring} but BERT is used as encoder and decoder instead of LSTM;
    \item[v]\textbf{BERT-LSTM + Attention:} This has only task-level supervision and rationales are extracted based on attention score. Glove embeddings are considered for \fever{} instead of \bert{} due to computational constraint;
    \item[vi]\textbf{BERT-LSTM + Simple Gradient:} Same as (v) but tokens are ranked based on gradients.
\end{enumerate}
In order to evaluate the performance of our MTL approach on either task, we also adapt models aiming to one task, i.e. the \bert{} with a single explainer or a single classifier, as baselines.

\subsection{Metrics} 
In earlier work~\citet{lei2016rationalizing,deyoung2019eraser}, the \hard and \soft explanation models are evaluated under six metrics in total.

\textbf{Macro F1} For both \hard~and \soft~selection the \textbf{Macro F1} is used to evaluate the performance of the classifier.

\textbf{Token F1} The token-wise F1 is used in \hard selection to describe concordance of explainer's output with human annotation.

\textbf{IOU (Intersection-Over-Union) F1.} is also used for \hard selection models. It considers a prediction as true positive if its token-wise IOU (length of overlap divided by length of union) is larger than a threshold (we choose the threshold to be $0.5$ to be consistent with the measurements in prior works).

\textbf{AUPRC.} or area under the precision-recall curve is used for the soft selection models. Since for soft-annotation for each token is assigned with a ranking score (sometimes probability of being rationale).

\textbf{Comprehensiveness and Sufficiency.}
Proposed by~\citet{deyoung2019eraser} the~\textbf{comprehensiveness} of a rationale $r_{ij}$ on instance $i$ and class $j$ is defined as $\mbox{comprehensiveness}(r)=\hat{p}_{ij}-\tilde{p}_{ij}$, where $\hat{p}_{ij}$ is model's prediction on the original input, and $\tilde{p}_{ij}$ is prediction over the input where the rationale $r_{ij}$ is stripped. 
~\textbf{Sufficiency} on the other hand is defined as the complement of the comprehensiveness, $\mbox{sufficiency}=\hat{p}_{ij}-\bar{p}_{ij}$, where $\bar{p}_{ij}$ is the predicted probability using \emph{only} rationale $r_{ij}$. They are provided as metrics for \soft selection models.


\subsection{Datasets}
We consider three diverse language tasks for our evaluation.

\textbf{\movie}~\citet{zaidan2007using,zaidan2008modeling}. One of the original datasets providing extractive rationales, the movies dataset has \textit{pos}itive or \textit{neg}ative sentiment labels on movie reviews. As the included rationale annotations are not necessarily comprehensive (i.e., annotators were not asked to mark \emph{all} text supporting a label), we collect a comprehensive evaluation set on the final fold of the original dataset~\citet{pang2004sentimental}

\textbf{ \fever}~\citet{Thorne18Fever} (short
for Fact Extraction and VERification) is a fact-checking dataset. 
The task is to verify claims from textual sources. 
In particular, each claim is to be classified as \textit{supported}, \textit{refuted} or \textit{not enough information} with reference to a collection of potentially relevant source texts.  
We follow the setup of ~\citet{deyoung2019eraser} who restrict this dataset to \textit{supported} or \textit{refuted}.

\textbf{ \multirc}~\citet{khashabi2018looking}. This is a reading comprehension dataset composed of questions with multiple correct answers that by construction depend on information from multiple sentences. In \multirc{}, each Rationale is associated with a question, while answers are independent of one another. We convert each rationale/question/answer triplet into an instance within our dataset. Each answer
candidate then has a label of \textit{True} or \textit{False}.

The train/val/test set are kept the same as provided by ~\citet{deyoung2019eraser}. The other datasets either contains over-length documents thus are not yet considered in this work.


==> trash bin/06.results.backup.tex <==
\section{Results}
\label{sec:results}
This section presents the research results based on the questions formulated in the previous section.

 
\begin{table}[tb]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
        & \textbf{Macro F1} & \textbf{IOU F1} & \textbf{token F1} \\
    \hline
    \textbf{\movie}\\
    \citet{lei2016rationalizing} & 0.914 & 0.124 & 0.285\\
    \citet{lei2016rationalizing}(u) &\textbf{0.920} & 0.012 & \textbf{0.322}\\
    \citet{lehman2019inferring} & 0.738 & 0.057 & 0.121\\
    Bert-To-Bert & 0.864 & 0.067 & 0.115\\
    \hline
    \methodindv{} ($\lambda = 5.0$) & 0.869 & \textbf{0.314} & 0.278\\
    %\methodindv ($\lambda=1.0$) & 0.859 & \textbf{0.198} & 0.240\\
    % \methodspan ($\lambda=0.1$) & 0.894 & 0.018 & 0.206\\
    \hline
    % \hline
    \\
    \textbf{\fever}\\
    \citet{lehman2019inferring} & 0.687 & 0.571 & 0.554\\
    Bert-To-Bert & 0.850 & \textbf{0.817} & \textbf{0.796}\\
    \hline
    \methodindv ($\lambda=5.0$) & \textbf{0.914} & 0.753 & 0.732\\
    % \methodspan ($\lambda=0.2$) & 0.902 & 0.726 & 0.664\\
    \hline
    % \hline
    \\
    \textbf{\multirc}\\
    \citet{lei2016rationalizing} & 0.655 & 0.271 & 0.456\\
    \citet{lei2016rationalizing}(u) & 0.652 & 0.000 & 0.000\\
    \citet{lehman2019inferring} & 0.592 & 0.151 & 0.152\\
    Bert-To-Bert & 0.610 & \textbf{0.419} & 0.402\\
    \hline
    \methodindv ($\lambda=2.0$) & \textbf{0.726} & 0.363 & \textbf{0.603}\\
    % \methodspan ($\lambda=0.05$) & 0.689 & 0.254 & 0.382\\
    % \methodspan ($\lambda=0.1$) & 0.658 & 0.254 & 0.404\\
 \bottomrule
    % \hline
    
    \end{tabular}
    }
    \caption{Performance of \textbf{Hard Selection} baseline models, and the proposed MTL approaches (\methodindv{}, and \methodspan{}) over three datasets. Metrics are taken from the ERASER~\citet{deyoung2019eraser}.}
    \label{table:task_explanation_result_hard}
    \vspace{-5mm}
\end{table}

\begin{table*}[tb]
    
    \centering
    \begin{tabular}{lcccc}
    \toprule
        & \textbf{Macro F1} & \textbf{AUPRC} & \textbf{Comprehensiveness$\uparrow$} & \textbf{Sufficiency$\downarrow$}\\
    \hline
    \textbf{\movie}\\
    BERT-LSTM + Attention & \textbf{0.974} & 0.467  & 0.091 & \textbf{0.035}\\
    BERT-LSTM + Simple Gradient & \textbf{0.974} & 0.441 & 0.113 & 0.052\\
    \hline
    \methodindv 
     ($\lambda=5.0$) 
    & 0.869 & \textbf{0.470} & \textbf{0.287} & 0.170\\
    % \methodspan 
    %  ($\lambda=0.1$) 
    % & 0.894 &-& 0.055 & 0.244\\
    
    
    \hline
    \\
    \textbf{\fever}\\
    GloVe-LSTM + Attention & 0.660 & 0.617 & -0.011 & 0.129\\
    GloVe-LSTM + Simple Gradient & 0.660 & 0.271 & 0.070 & 0.077\\
    \hline
    \methodindv
     ($\lambda=5.0$) 
    & \textbf{0.914} & \textbf{0.836} & \textbf{0.151} & \textbf{0.068}\\
    % \methodspan
    %  ($\lambda=0.2$) 
    % & 0.902 & - & 0.146 & 0.129\\
    
    \hline
    \\
    \textbf{\multirc}\\
    BERT-LSTM + Attention & 0.655 & 0.240 & 0.145 & 0.085\\
    BERT-LSTM + Simple Gradient & 0.655 & 0.224 & \textbf{0.164} & 0.079\\
    \hline
    \methodindv 
     ($\lambda=2.0$) 
    & \textbf{0.726} & \textbf{0.695} & 0.157 & \textbf{0.031}\\
    %\methodspan
    % ($\lambda=0.05$) 
    %& 0.689 & - & 0.080 & 0.151\\
   \bottomrule

    \end{tabular}
    %}
    \caption{Performance of \textbf{soft-selection} baseline models, and the proposed MTL approaches (\methodindv{}, and \methodspan{}) over three datasets. Metrics are taken from the ERASER~\citet{deyoung2019eraser}.}
    \label{table:task_explanation_result_soft}
\end{table*}

\noindent\textbf{How effective is the Multi-Task Learning (MTL) framework for joint task and explanation learning?}
In this section, we first evaluate the performance of the proposed MTL framework. Tables~\ref{table:task_explanation_result_hard} and~\ref{table:task_explanation_result_soft} report the performance of the baselines, \methodindv{}, and \methodspan{}. As mentioned earlier, baseline models are broadly of two categories (hard and soft selection) based on their rationale selection process. Table~\ref{table:task_explanation_result_hard} reports the result for hard rationale selection based baselines, \methodindv{}, and \methodspan. Performance of these baselines are measured in terms of \textbf{macro-avg-F1}, \textbf{IOU F1}, and \textbf{token F1} because such models contain rationale level supervision. On the other hand, results for soft-selection approaches are presented in Table~\ref{table:task_explanation_result_soft}. These models are trained only on task level data and do not have any explicit rationale level supervision. Hence, \textbf{Macro F1}, \textbf{AUPRC}, \textbf{Comprehensiveness}, and \textbf{Sufficiency} metrics are computed for these baselines.

It is evident from Table~\ref{table:task_explanation_result_hard} that none of the methods perform consistently well across all the three metrics. However, \methodindv{} efficiently handles the trade-off between task prediction and rationale selection and keeps a consistent balance among all the three metrics. \methodindv{} shows better task performance (macro-avg-F1) for \fever{} and \multirc{} without significant drop in IOU F1 and token F1.

Table~\ref{table:task_explanation_result_soft} highlights the effect of multi-task learning framework. \methodindv{} performs consistently well both in terms of task and rationale selection metrics. Higher value of  AUPRC  indicates that better choice of threshold of per token rationale prediction can help in improving explainability. Higher value of comprehensiveness indicates that \methodindv{} selects the correct rationales that are responsible for accurate task label prediction i.e., task performance drops significantly without these tokens. Low value of sufficiency also supports the fact i.e., it is an indication that model is able to learn the task well only based on those tokens. For \movie, BERT-LSTM + Attention is able to identify rationales well (low sufficiency) and high value of AUPRC indicates that rationales are in accordance with human annotated ones. However, the low value of comprehensiveness reveals that the model can still learn without those rationales that might lead to the option that attention based selections are not always rationales~\citet{jain2019attention}.
On the other hand, \methodindv{} ensures that the rationales learned are in accordance with human rationales and the model performance significantly drops without those tokens. 
It fits with our objective that the models should be interpretable by design. However, \methodindv{} achieves high comprehensiveness but sufficiency is higher than the baselines. 
This suggests that our method is able to retrieve rationale tokens quite well but those are not sufficient to learn the task i.e., it fails to capture some rationale tokens. However, it is able to maintain a balance between task and rationale selection. 



\textbf{What are the task-explanation performance trade-offs in an MTL framework?}



\begin{table}[tb]
    \centering
    \resizebox{\linewidth}{!}{
    % \begin{tabular}{lccc}
    % \toprule
    %           & \textbf{TASK} accuracy & \textbf{TASK Macro F1} & \textbf{EXP}-token-F1  \\
    %     \hline
    %      \textbf{\movie}&&\\
    %      \textsc{TASK} & 0.894 & 0.894 & -\\
    %      \textsc{Token} - EXP & - & - & 0.335 \\
    %      %\textsc{Span} - EXP & - & - & 0.315 \\
    %      \methodindv($\lambda=5.0$) & 0.879 & 0.869 & 0.324\\
    %      %\methodspan($\lambda=0.1$) & 0.889 & & 0.140\\
    %      \hline
    %      \\
    %      \textbf{\fever}\\ 
    %      \textsc{TASK} & 0.917 & 0.916 & -\\
    %      \textsc{Token} - EXP & - & - & 0.820 \\
    %      %\textsc{Span} - EXP & - & - & 0.449 \\
    %      \methodindv($\lambda=5.0$) & 0.914 & 0.914 & 0.831\\
    %      %\methodspan($\lambda=0.2$) & 0.902 && 0.729\\
    %      \hline
    %      \\
    %      \textbf{\multirc}&&\\
    %      \textsc{TASK} & 0.721 & 0.708 & - \\
    %      \textsc{Token} - EXP & - & - & 0.839 \\
    %      %\textsc{Span} - EXP & - & - & 0.424 \\
    %      \methodindv($\lambda=2.0$) & 0.730 & 0.726 & 0.599 \\
    %      %\methodspan($\lambda=0.1$) & 0.692 & & 0.290\\
    % \bottomrule
    % \end{tabular}
        \begin{tabular}{lcc}
    \toprule
              & \textbf{TASK Macro F1} & \textbf{EXP}-token-F1  \\
        \hline
         \textbf{\movie}&&\\
         \textsc{TASK} & 0.894 & -\\
         \textsc{Token} - EXP &  - & 0.335 \\
         \methodindv($\lambda=5.0$) &  0.869 & 0.324\\
         \hline
         \\
         \textbf{\fever}\\ 
         \textsc{TASK} & 0.916 & -\\
         \textsc{Token} - EXP & - & 0.820 \\
         \methodindv($\lambda=5.0$) & 0.914 & 0.831\\
         \hline
         \\
         \textbf{\multirc}&&\\
         \textsc{TASK} & 0.708 & - \\
         \textsc{Token} - EXP & - & 0.839 \\
         \methodindv($\lambda=2.0$) & 0.726 & 0.599 \\
    \bottomrule
    \end{tabular}
    \vspace{-3cm}
    }
    \caption{{\bf The individual \textsc{TASK} and EXPLANATION (EXP)  performance of MTL based models. \textbf{EXP}-token-F1 represents the token-wise rationale F1 for the sub-token inputs of \bert{}(sequence length $\leq512$). Metrics are taken from the ERASER~\citet{deyoung2019eraser}.}}
    \label{table:mtl}
    \vspace{-3mm}
\end{table}

In this part, our objective is to verify the effect of rationales on task performance and vice-versa. The motivation behind MTL is that there should not be any significant drop in task accuracy because of the explanation part i.e., it can effectively handle the task-explanation trade-off and both the task and explanation can take benefit from each other. Table~\ref{table:mtl} shows the effect of task and explanation based training scenarios. This trend is quite evident for \fever{} and \movie{}. In general, the explanation part works as a regularizer to improve the task prediction and avoid overfitting. A detailed analysis reveals that \methodspan{} has to learn a lot of parameters and performs worse than \methodindv{} due to overfitting issue. We leave the task of learning the impact of precise or general explanation structures on model performance as a future work.



\noindent\textbf{What impact does $\lambda$ have on task and explanation performance?}

\begin{figure}[tb] 
  \centering 
  \subfigure[\textbf{Classification Macro Average F1}]{ 
    \label{fig:subfig:acc}
  
    \includegraphics[width=0.48\columnwidth]{figs/task_f1.pdf}}

  \subfigure[\textbf{Explanation Macro F1}]{ 
    \label{fig:subfig:macro_f1}
    \includegraphics[width=0.48\columnwidth]{figs/hard_exp_metric.pdf}}

    \caption{Performance variation of task (a) and explanation (macro token/IOU-F1) (b) of \methodindv{} with $\lambda$ (log-scale) on the first 10\% \fever{} dataset. Here we can see the obvious contradiction between classification and explanation along the $\lambda$ increases}
    
  \label{fig:lambda-sweep_1} 
\end{figure}


\begin{figure}[tb] 
  \centering 

  \subfigure[\textbf{Comprehensiveness and Sufficiency}]{ 
    \label{fig:subfig:cs}
    \includegraphics[width=0.48\columnwidth]{figs/comp_suff.pdf}}

  \subfigure[\textbf{Explanation AUPRC}]{ 
  \label{fig:subfig:auprc}
    \includegraphics[width=0.48\columnwidth]{figs/auprc.pdf}}
    \caption{{\bf Variation of comprehensiveness and sufficiency (a) and AUPRC of explanations (b) of \methodindv{} with $\lambda$ (log-scale) on the first 10\% \fever{} dataset.}}
    
    \label{fig:lambda-sweep_2} 
%   \vspace{-3mm}
\end{figure}


All the results reported so far are based on the $\lambda$ value that shows best performance on the validation set. In this part, we try to elaborate the effect of $\lambda$-sweep on both task and explanation. We observe an opposite trend in task and explanation i.e., the performance of the task decreases and explanation increases with the increased value of $\lambda$. In this part, we highlight the effect of $\lambda$-sweeping on the head 10\% \fever{} dataset\footnote{Similar trend is observed for other datasets.}. Figure~\ref{fig:lambda-sweep_1} (a) and (b) clearly reflect the contrasting effect. The task F1 score goes on decreasing while explanation scores (IOU F1, token F1) improve with increment of  $\lambda$. Task accuracy deteriorates rapidly after $\lambda\geq50$. Figure~\ref{fig:lambda-sweep_2}(d) supports the same trend i.e., rationale token AUPRC goes on increasing with $\lambda$. Slightly different trend is observed for comprehensiveness($\uparrow$) and sufficiency($\downarrow$). There is no monotonic increment and decrement in the performance with the variation in $\lambda$. Performance reaches a peak point within an interval and subsequently it starts to deteriorate. Hence, a careful selection $\lambda$ is required to effectively handle the trade-off between task and rationales.


% The values of $\lambda$'s in the table \ref{table:mtl} as well as \ref{table:downstream} are selected by increasing it in log-scale and select the one brings the best performance on the evaluation set. Intuitively, the greater $\lambda$ is, the more the final performance tilts to the explanation task, i.e. the performance of classification deteriorates and that of explanation improves. The figures in \ref{fig:lambda-sweep} verifies this hypothesis. These figures are based on results of $\lambda$-sweeping on the head 10\% of the \fever~dataset. The sub-figure \ref{fig:subfig:acc} indicates descending of classification accuracy along with increment of $\lambda$, while for the explanation metrics such as IOU-F1, Token-F1~\ref{fig:subfig:macro_f1} and AUPRC~\ref{fig:subfig:auprc} it is totally opposite. From the figure we can also tell that the accuracy rapidly deteriorates especially when $\lambda\geq50$, and the IOU- and Token-F1 keep on increasing tremendously before $\lambda\leq 1$. For the comprehensiveness (the higher the better) and sufficiency (the lower the better)~\ref{fig:subfig:cs} some other patterns emerge. It seems that for the comprehensiveness there is an optimal interval of $\lambda$, where it performs well, while the sufficiency decreases all the way through. Taking all those metrics into consideration, we need to find a $\lambda$ which induces high classification accuracy, high comprehensiveness, low sufficiency and high on F1-s and AUPRC, therefore $\lambda=5$ could be a good choice. The choosing of optimal $\lambda$-s for other structures and/or datasets follows analogy procedure. To save the page we leave other $\lambda$-sweeping figures to the appendix.



% \if 0
% \begin{figure*}[tb] 
%   \centering 
%   \subfigure[Classification Macro Average F1]{ 
%     \label{fig:subfig:acc}
%     \includegraphics[width=0.48\linewidth]{figs/lambda_sweep/fever_gru_val_train_on_portion_0_1_macro_avg_f1.png}}
%   \subfigure[Comprehensiveness and Sufficiency]{ 
%     \label{fig:subfig:cs}
%     \includegraphics[width=0.48\linewidth]{figs/lambda_sweep/fever_gru_val_train_on_portion_0_1_cs.png}}
%   \subfigure[Explanation Macro F1]{ 
%     \label{fig:subfig:macro_f1}
%     \includegraphics[width=0.48\linewidth]{figs/lambda_sweep/fever_gru_val_train_on_portion_0_1_iou_token_f1.png}}
%   \subfigure[Explanation AUPRC]{ 
%     \label{fig:subfig:auprc}
%     \includegraphics[width=0.48\linewidth]{figs/lambda_sweep/fever_gru_val_train_on_portion_0_1_auprc.png}}
%   \caption{Performance of \textit{cls} and \textit{exp} task in \methodindv w.r.t. 6 metrics on log-scale variation of $\lambda$ on the top 10\% data of~\fever. Horizontal lines and curves sharing same line type in each sub-figure correspond to the same metric, where the horizontal lines are the highest (for sufficiency the lowest) scores of each metrics out of all baseline models.}
%   \label{fig:lambda-sweep} 
% \end{figure*}
% \fi


% \begin{table*}
% \label{table:task_performance}
%     \centering
%     \begin{tabular}{l|c|c|c|c}
%              & \movie & \multirc & \fever~\\
%              \hline
%         \gru  - CLS&&&\\ 
%         \elmo - CLS&&&\\
%         \bert - CLS& 0.886 & 0.908 & 0.707 & 0.908\\
%         \bert - MTL & 0.XXX & 0.XXX & 0.XXX & 0.819\\
%     \end{tabular}
%     \caption{Task accuracy of three different models (task only)}
% \end{table*}
% Along side the classification, we need also to annotate explicit evidence supporting this classification on the input sentence. Conditions used in filtering objective twitters in \semsent{} (final.polarity\_in\_dataset!='neutral')
%               \& (final.subjectivity>0)
%               \& ((abs(final.polarity\_textblob) > 0.1))=>10196 out of 30466 instances passed this subjectivity test, where 6530 are used for testing, 699 for dev, 680 for devtest and 2061 fro training.


% \begin{table*}
% \label{table:task_performance}
%     \centering
%     \begin{tabular}{l|c|c|c|c}
%              & \imdb & \semsent & \semirony & \zaidan \\
%              \hline
%         \gru  - EXP &&&\\ 
%         \elmo - EXP &&&\\
%         \bert - EXP & 0.XXX & 0.XXX & 0.XXX & 0.941\\
%         \bert - MTL & 0.XXX & 0.XXX & 0.XXX & 0.931\\
%     \end{tabular}
%     \caption{Explanation Accuracy of three different models}
% \end{table*}

% bert with length of sequence == 128
%------------------------
% bert@ACL IMDB:
% {'auc': 0.88628,
%  'eval_accuracy': 0.88628,
%  'f1_score': 0.8865658,
%  'false_negatives': 1390.0,
%  'false_positives': 1453.0,
%  'global_step': 2343,
%  'loss': 0.4798463,
%  'precision': 0.8843429,
%  'recall': 0.8888,
%  'true_negatives': 11047.0,
%  'true_positives': 11110.0}
%-----------------------------
%bert @ imdb length == 512
% {'auc': 0.93851995,
%  'eval_accuracy': 0.93852,
%  'f1_score': 0.9382606,
%  'false_negatives': 821.0,
%  'false_positives': 716.0,
%  'loss': 0.35001868,
%  'precision': 0.94223475,
%  'recall': 0.93432,
%  'true_negatives': 11784.0,
%  'true_positives': 11679.0,
%  'global_step': 9375}
 %---------------------------
 % bert@semeval 2016 sentiment seq_len=128
%  {'auc': 0.87515986,
%  'eval_accuracy': 0.90816325,
%  'f1_score': 0.93506485,
%  'false_negatives': 255.0,
%  'false_positives': 690.0,
%  'global_step': 494,
%  'loss': 0.37832594,
%  'precision': 0.9079263,
%  'recall': 0.9638759,
%  'true_negatives': 2541.0,
%  'true_positives': 6804.0}
%bert@semeval2016 sentiment seq_len=512
% {'auc': 0.8695189,
%  'eval_accuracy': 0.90767735,
%  'f1_score': 0.93525964,
%  'false_negatives': 197.0,
%  'false_positives': 753.0,
%  'loss': 0.4629555,
%  'precision': 0.9011162,
%  'recall': 0.9720924,
%  'true_negatives': 2478.0,
%  'true_positives': 6862.0,
%  'global_step': 1978}
%-----------------------------
% bert@semeval 2018 irony seq_len=128
% {'auc': 0.70947224,
%  'eval_accuracy': 0.70790815,
%  'f1_score': 0.6607407,
%  'false_negatives': 88.0,
%  'false_positives': 141.0,
%  'global_step': 357,
%  'loss': 0.8956044,
%  'precision': 0.61263734,
%  'recall': 0.7170418,
%  'true_negatives': 332.0,
%  'true_positives': 223.0}
%---------------------
%bert@semeval 2018 irony seq_len=512
% {'auc': 0.7169602,
%  'eval_accuracy': 0.71428573,
%  'f1_score': 0.66961646,
%  'false_negatives': 84.0,
%  'false_positives': 140.0,
%  'loss': 1.2306125,
%  'precision': 0.6185286,
%  'recall': 0.7299035,
%  'true_negatives': 333.0,
%  'true_positives': 227.0,
%  'global_step': 1431}
% ---------------------------------
% bert@zaidan07
% {'auc': 0.9079837,
%  'eval_accuracy': 0.90833336,
%  'f1_score': 0.9115281,
%  'false_negatives': 13.0,
%  'false_positives': 20.0,
%  'global_step': 135,
%  'loss': 0.18267174,
%  'precision': 0.8947368,
%  'recall': 0.92896175,
%  'true_negatives': 157.0,
%  'true_positives': 170.0}
%--------------------------------------
%--------------------------------------
%bert with max_seq_length=512
% {'auc': 0.99397594,
%  'eval_accuracy': 0.99444443,
%  'f1_score': 0.99487174,
%  'false_negatives': 0.0,
%  'false_positives': 2.0,
%  'loss': 0.027238758,
%  'precision': 0.9897959,
%  'recall': 1.0,
%  'true_negatives': 164.0,
%  'true_positives': 194.0,
%  'global_step': 540}.0}
%---------------------------------------
%---------------------------------------
%gru on zaidan07 with max_seq_length=128, batch_size=64, learning_rate=1e-2,epoch=15,num_gru_units=128, embedding_size=100
% {'auc': 0.81780726,
%  'eval_accuracy': 0.82222223,
%  'f1_score': 0.7974683,
%  'false_negatives': 43.0,
%  'false_positives': 21.0,
%  'loss': 0.4920561,
%  'precision': 0.85714287,
%  'recall': 0.74556214,
%  'true_negatives': 170.0,
%  'true_positives': 126.0,
%  'global_step': 42}
%-----------------------------
%gru on imdb 
% {'auc': 0.77712005,
%  'eval_accuracy': 0.77712,
%  'f1_score': 0.76419795,
%  'false_negatives': 3471.0,
%  'false_positives': 2101.0,
%  'global_step': 732,
%  'loss': 0.5287146,
%  'precision': 0.8112309,
%  'recall': 0.72232,
%  'true_negatives': 10399.0,
%  'true_positives': 9029.0}
%-----------------------------------------
%gru on SemEval16(sent)
% {'auc': 0.5,
%  'eval_accuracy': 0.68600583,
%  'f1_score': 0.81376445,
%  'false_negatives': 0.0,
%  'false_positives': 3231.0,
%  'loss': 0.6292327,
%  'precision': 0.68600583,
%  'recall': 1.0,
%  'true_negatives': 0.0,
%  'true_positives': 7059.0,
%  'global_step': 154}
%------------------------------
%gru on SemEval18(sarcasm)max_seq_len=64
% {'auc': 0.6604046,
%  'eval_accuracy': 0.6619898,
%  'f1_score': 0.605067,
%  'false_negatives': 108.0,
%  'false_positives': 157.0,
%  'loss': 0.6578578,
%  'precision': 0.5638889,
%  'recall': 0.65273315,
%  'true_negatives': 316.0,
%  'true_positives': 203.0,
%  'global_step': 745}
%----------------------------------------
%----------------------------------------
%bert on ration(seq) zaidan07
%val_acc: 0.9411


==> trash bin/06.results.tex <==
\section{Results}
% [下午2:21] Avishek Anand
%     so our design space is the following hard selection approaches 1) MTL + TASK, 2) EXP + TASK, 3) Competitors....EXP is when you use BERT only to optimize the explanation task and do not consider the task like in MTL
% 已编辑​[下午2:22] Avishek Anand
%     so RQ1: how does 1) compare vs 2) for Task performance 
% ​[下午2:23] Avishek Anand
%     RQ2: How does explanations from MTL (2) compare against only predicting the explanations (2)



\label{sec:results}
This section presents the research results based on the questions formulated in the previous section.

% \begin{table}[]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lccc}
%         \toprule
%             & \textbf{Macro F1} & \textbf{IOU F1} & \textbf{Token F1}\\
%         \hline
%         \textbf{\movie}\\
%         \citet{lei2016rationalizing} & 0.914 & 0.124 & 0.285\\
%         \citet{lei2016rationalizing}(u) &\textbf{0.920} & 0.012 & \textbf{0.322}\\
%         \citet{lehman2019inferring} & 0.738 & 0.057 & 0.121\\
%         Bert-To-Bert & 0.864 & 0.067 & 0.115\\
%         \hline
%         \mtlhard($\lambda=5.0$) & 0.885 & 0.109 & 0.169\\
%         \exptask & 0.980 & 0.140 & 0.217\\
%         \hline\\
%         \textbf{\fever}\\
%         \citet{lehman2019inferring} & 0.687 & 0.571 & 0.554\\
%         Bert-To-Bert & 0.850 & \textbf{0.817} & \textbf{0.796}\\
%         \hline
%         \mtlhard($\lambda=20.0$) & 0.894 & 0.751 & 0.735\\
%         \exptask & 0.920 & 0.749 & 0.739\\
%         \hline\\
%         \textbf{\multirc}\\
%         \citet{lei2016rationalizing} & 0.655 & 0.271 & 0.456\\
%         \citet{lei2016rationalizing}(u) & 0.652 & 0.000 & 0.000\\
%         \citet{lehman2019inferring} & 0.592 & 0.151 & 0.152\\
%         Bert-To-Bert & 0.610 & \textbf{0.419} & 0.402\\
%         \hline
%         \mtlhard($\lambda=2.0$) & 0.719 & 0.388 & 0.573\\
%         \exptask & 0.761 & 0.397 & 0.597\\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Task and explanation performance of hard models}
%     \label{tab:hard_task_performance}
% \end{table}

% % \begin{table}[tb]
% %     \centering
% %     \resizebox{\linewidth}{!}{
% %     \begin{tabular}{lccc}
% %     \toprule
% %         & \textbf{Macro F1} & \textbf{IOU F1} & \textbf{token F1} \\
% %     \hline
% %     \textbf{\movie}\\
% %     \citet{lei2016rationalizing} & 0.914 & 0.124 & 0.285\\
% %     \citet{lei2016rationalizing}(u) &\textbf{0.920} & 0.012 & \textbf{0.322}\\
% %     \citet{lehman2019inferring} & 0.738 & 0.057 & 0.121\\
% %     Bert-To-Bert & 0.864 & 0.067 & 0.115\\
% %     \hline
% %     \methodindv{} ($\lambda = 5.0$) & 0.869 & \textbf{0.314} & 0.278\\
% %     %\methodindv ($\lambda=1.0$) & 0.859 & \textbf{0.198} & 0.240\\
% %     % \methodspan ($\lambda=0.1$) & 0.894 & 0.018 & 0.206\\
% %     \hline
% %     % \hline
% %     \\
% %     \textbf{\fever}\\
% %     \citet{lehman2019inferring} & 0.687 & 0.571 & 0.554\\
% %     Bert-To-Bert & 0.850 & \textbf{0.817} & \textbf{0.796}\\
% %     \hline
% %     \methodindv ($\lambda=5.0$) & \textbf{0.914} & 0.753 & 0.732\\
% %     % \methodspan ($\lambda=0.2$) & 0.902 & 0.726 & 0.664\\
% %     \hline
% %     % \hline
% %     \\
% %     \textbf{\multirc}\\
% %     \citet{lei2016rationalizing} & 0.655 & 0.271 & 0.456\\
% %     \citet{lei2016rationalizing}(u) & 0.652 & 0.000 & 0.000\\
% %     \citet{lehman2019inferring} & 0.592 & 0.151 & 0.152\\
% %     Bert-To-Bert & 0.610 & \textbf{0.419} & 0.402\\
% %     \hline
% %     \methodindv ($\lambda=2.0$) & \textbf{0.726} & 0.363 & \textbf{0.603}\\
% %     % \methodspan ($\lambda=0.05$) & 0.689 & 0.254 & 0.382\\
% %     % \methodspan ($\lambda=0.1$) & 0.658 & 0.254 & 0.404\\
% %  \bottomrule
% %     % \hline
    
% %     \end{tabular}
% %     }
% %     \caption{Performance of \textbf{Hard Selection} baseline models, and the proposed MTL approaches (\methodindv{}, and \methodspan{}) over three datasets. Metrics are taken from the ERASER~\citet{deyoung2019eraser}.}
% %     \label{table:task_explanation_result_hard}
% %     \vspace{-5mm}
% % \end{table}

% \begin{table*}[]
%     \centering
%     %\resizebox{\linewidth}{!}{
%     \begin{tabular}{lcc}
%     \toprule
%                     & explanation only & without explanation \\
%         \hline
%         \textbf{\movie}\\
%         \exptask &  \textbf{0.980} & 0.675\\
%         \mtlhard($\lambda=5.0$) & 0.960 & \textbf{0.487}\\
%         \human & 0.899 & 0.523\\
%         \hline\\
%         \textbf{\fever}\\
%         \exptask & 0.920 & \textbf{0.803}\\
%         \mtlhard($\lambda=20.0$) & 0.913 & 0.819\\
%         \human & \textbf{0.921} & 0.827\\
%         \hline\\
%         \textbf{\multirc}\\
%         \exptask & 0.761 & \textbf{0.623}\\
%         \mtlhard($\lambda=2.0$) & \textbf{0.913} & 0.819\\
%         \human & 0.759 & 0.633\\
%     \bottomrule
%     \end{tabular}
%     %}
%     \caption{The explanation quality of hard models}
%     \label{tab:hard_models_exp_quality}
% \end{table*}

% \begin{table*}[tb]
%     \centering
%     \begin{tabular}{lcccc}
%     \toprule
%         & \textbf{Macro F1} & \textbf{AUPRC} & \textbf{Comprehensiveness$\uparrow$} & \textbf{Sufficiency$\downarrow$}\\
%     \hline
%     \textbf{\movie}\\
%     BERT-LSTM + Attention & \textbf{0.974} & \textbf{0.467}  & 0.091 & \textbf{0.035}\\
%     BERT-LSTM + Simple Gradient & \textbf{0.974} & 0.441 & 0.113 & 0.052\\
%     \hline
%     \mtlsoft($\lambda=50.0$) & 0.88 & 0.420 & \textbf{0.385} & 0.163\\
%     \hline\\
%     \textbf{\fever}\\
%     GloVe-LSTM + Attention & 0.660 & 0.617 & -0.011 & 0.129\\
%     GloVe-LSTM + Simple Gradient & 0.660 & 0.271 & 0.070 & 0.077\\
%     \hline
%     \mtlsoft($\lambda=5.0$) & \textbf{0.914} & \textbf{0.836} & \textbf{0.151} & \textbf{0.068}\\
%     \hline\\
%     \textbf{\multirc}\\
%     BERT-LSTM + Attention & 0.655 & 0.240 & 0.145 & 0.085\\
%     BERT-LSTM + Simple Gradient & 0.655 & 0.224 & \textbf{0.164} & 0.079\\
%     \hline
%     \mtlsoft($\lambda=2.0$) & \textbf{0.726} & \textbf{0.695} & 0.157 & \textbf{0.031}\\
%     \bottomrule
%     \end{tabular}
%     \caption{Performance of \textbf{soft-selection} baseline models.}
%     \label{table:task_explanation_result_soft}
% \end{table*}


\noindent\textbf{What are the task-explanation performance trade-offs in the MTL framework?}
At first we try to elaborate the effect of $\lambda$-sweep on both task and explanation for both \mtlhard and \mtlsoft. In general we observe an opposite trend in task and explanation i.e., the performance of the task decreases and of explanation increases with the increased value of $\lambda$. In this part, we highlight the effect of $\lambda$-sweeping on the head 10\% \fever{} dataset\footnote{Similar trend is observed for other datasets.}. Figure~\ref{fig:lambda-sweep_1} (a) and (b) clearly reflect the contrasting effect. 


\begin{figure}[tb] 
  \centering 
  \subfigure[\textbf{Classification Macro Average F1}]{ 
    \label{fig:subfig:acc}
    \includegraphics[width=0.48\columnwidth]{figs/task_f1.pdf}}

  \subfigure[\textbf{Explanation Macro F1}]{ 
    \label{fig:subfig:macro_f1}
    \includegraphics[width=0.48\columnwidth]{figs/hard_exp_metric.pdf}}
    \caption{\bf Performance variation of task (a) and explanation (macro token/IOU-F1) (b) of \mtlhard with $\lambda$ (log-scale) on the first 10\% \fever{} dataset.}
  \label{fig:lambda-sweep_1} 
\end{figure}


% \begin{figure}[tb] 
%   \centering 
%   \subfigure[\textbf{Comprehensiveness and Sufficiency}]{ 
%     \label{fig:subfig:cs}
%     \includegraphics[width=0.48\columnwidth]{figs/comp_suff.pdf}}

%   \subfigure[\textbf{Explanation AUPRC}]{ 
%   \label{fig:subfig:auprc}
%     \includegraphics[width=0.48\columnwidth]{figs/auprc.pdf}}
%     \caption{{\bf Variation of comprehensiveness and sufficiency (a) and AUPRC of explanations (b) of \mtlsoft with $\lambda$ (log-scale) on the first 10\% \fever{} dataset.}}
%     \label{fig:lambda-sweep_2} 
% %   \vspace{-3mm}
% \end{figure}

In this part, we try to elaborate the effect of $\lambda$-sweep on both task and explanation. We observe an opposite trend in task and explanation i.e., the performance of the task decreases and explanation increases with the increased value of $\lambda$. Specifically, we highlight the effect of $\lambda$-sweeping on the head 10\% \fever{} dataset\footnote{Similar trend is observed for other datasets.}. Figure~\ref{fig:lambda-sweep_1} (a) and (b) clearly reflect the contrasting effect. For the \mtlhard, the task macro F1 score of the classifier goes on decreasing while explanation scores (IOU F1, token F1) improve with increment of  $\lambda$. Task accuracy deteriorates rapidly after $\lambda\geq50$. For the \mtlsoft, the same trend, i.e., rationale token AUPRC goes on increasing and sufficiency($\downarrow$) goes decreasing with $\lambda$, is supported by Figure~\ref{fig:lambda-sweep_2}(a) and Figure~\ref{fig:lambda-sweep_2}(b). Slightly different trend is observed for comprehensiveness($\uparrow$). There is no monotonic increment in the performance with the variation of $\lambda$. Performance reaches a peak point within an interval and subsequently it starts to deteriorate. Hence, a careful selection $\lambda$ is required to effectively handle the trade-off between task and rationales. In order to decide best performing $\lambda$ values, we choose a single metric for the explainer in either \mtlhard and \mtlsoft respectively along with their task performance. In \mtlhard we choose the token F1 and in \mtlsoft the AUPRC to represent the explainer's performance. The optimal $\lambda$s, as presented in following tables, are decided by the summation of them.


\noindent\textbf{How is the classification task performance of the \mtlhard?}
A hard-selection model defined in the ERASER work~\citet{deyoung2019eraser} follows a 2-tier schemata. The first tier extracts the explanations(evidences) from the input text at first, then a tier 2 classifier is trained on such evidences only. Our MTL model can also serves as a hard-selection model, named as \mtlhard, since it predicts binary token rationality together with its classification task. The comparison of classification task performance of our \mtlhard with other competitors in the ERASER work is presented in the table~\ref{tab:hard_task_performance}. We also adopt a 2-tier model as the baseline, where there is no MTL involved, i.e., in the tier 1 the \bert+explainer only extracts evidences, while the tier-2 model is a simple \bert+classifier.


\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
        \toprule
            & \textbf{Macro F1} & \textbf{IOU F1} & \textbf{Token F1}\\
        \hline\\
        \textbf{\movie}\\
        \citet{lei2016rationalizing} & 0.914 & 0.124 & 0.285 \\
        \citet{lei2016rationalizing}(u) & 0.920 & 0.012 & \textbf{0.322} \\
        \citet{lehman2019inferring} & 0.738 & 0.057 & 0.121 \\
        Bert-To-Bert & 0.864 & 0.067 & 0.115 \\
        \hline
        \mtlhard & \textbf{0.987} & 0.084 & 0.151 \\
        \mtltask & 0.889 & 0.084 & 0.151 \\
        \exptask & 0.880 & 0.116 & 0.197 \\
        \human & 0.899 & 1.0 & 1.0 \\
        \cls-only & 0.894 & - & - \\
        \hline
        \textbf{\fever}\\
        \citet{lehman2019inferring} & 0.687 & 0.571 & 0.554 \\
        Bert-To-Bert & 0.850 & \textbf{0.817} & \textbf{0.796} \\
        \hline
        \mtlhard & \textbf{0.952} & 0.751 & 0.735 \\
        \mtltask & 0.913 & 0.751 & 0.735 \\
        \exptask & 0.833 & 0.749 & 0.739 \\
        \cls-only & 0.916 & - & - & \\
        \human & 0.921 & 1.0 & 1.0 & \\
        \hline
        \textbf{\multirc}\\
        \citet{lei2016rationalizing} & 0.655 & 0.271 & 0.456 \\
        \citet{lei2016rationalizing}(u) & 0.652 & 0.000 & 0.000 \\
        \citet{lehman2019inferring} & 0.592 & 0.151 & 0.152 \\
        Bert-To-Bert & 0.610 & \textbf{0.419} & 0.402 \\
        \hline
        \mtlhard & \textbf{0.847} & 0.388 & 0.573 \\
        \mtltask & 0.744 & 0.388 & 0.573 \\
        \exptask & 0.706 & 0.397 & \textbf{0.597} \\
        \cls-only & 0.708 & - & - \\
        \human & 0.759 & 1.0 & 1.0 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Task and explanation performance of hard models}
    \label{tab:hard_task_performance}
\end{table}

% \begin{table*}[]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lccccc}
%         \toprule
%             & \textbf{Macro F1} & \textbf{IOU F1} & \textbf{Token F1} & \textbf{$\text{EXP}$} & \textbf{$\overline{\text{EXP}}$}\\
%         \hline\\
%         \textbf{\movie}\\
%         \citet{lei2016rationalizing} & 0.914 & 0.124 & 0.285 & - & - \\
%         \citet{lei2016rationalizing}(u) &\textbf{0.920} & 0.012 & \textbf{0.322} & - & - \\
%         \citet{lehman2019inferring} & 0.738 & 0.057 & 0.121 & - & - \\
%         Bert-To-Bert & 0.864 & 0.067 & 0.115 & - & - \\
%         \hline
%         \mtlhard($\lambda=5.0$) & 0.885 & 0.109 & 0.169 & - & 0.487 \\
%         MTL + Task($\lambda=5.0$) & 0.960 & 0.109 & 0.169 & - & - \\
%         \exptask & 0.980 & 0.140 & 0.217 & - & 0.675 \\
%         \human & 0.899 & 1.0 & 1.0 & - & 0.523 \\
%         \cls-only & 0.894 & - & - & - & - \\
%         \hline\\
%         \textbf{\fever}\\
%         \citet{lehman2019inferring} & 0.687 & 0.571 & 0.554 & - & - \\
%         Bert-To-Bert & 0.850 & \textbf{0.817} & \textbf{0.796} & - & - \\
%         \hline
%         \mtlhard($\lambda=20.0$) & 0.894 & 0.751 & 0.735 & 0.913 & 0.819 \\
%         \exptask & 0.920 & 0.749 & 0.739 & 0.920 & 0.803 \\
%         \cls-only & 0.916 & - & - & - & - \\
%         \human & - & 1.0 & 1.0 & 0.921 & 0.827 \\
%         \hline\\
%         \textbf{\multirc}\\
%         \citet{lei2016rationalizing} & 0.655 & 0.271 & 0.456 & - & - \\
%         \citet{lei2016rationalizing}(u) & 0.652 & 0.000 & 0.000 & - & - \\
%         \citet{lehman2019inferring} & 0.592 & 0.151 & 0.152 & - & - \\
%         Bert-To-Bert & 0.610 & \textbf{0.419} & 0.402 & - & - \\
%         \hline
%         \mtlhard($\lambda=2.0$) & 0.719 & 0.388 & 0.573 & 0.745 & 0.630 \\
%         \exptask & 0.761 & 0.397 & 0.597 & 0.761 & 0.623 \\
%         \cls-only & 0.708 & - & - & - & - \\
%         \human & - & 1.0 & 1.0 & 0.759 & 0.633 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Task and explanation performance of hard models}
%     \label{tab:hard_task_performance}
% \end{table*}

\textcolor{red}{describe task performance of \mtlhard}


% \textcolor{red}{RQ3: explanation quality \ref{tab:hard_models_exp_quality}}
% \begin{table*}[]
%     \centering
%     %\resizebox{\linewidth}{!}{
%     \begin{tabular}{lcc}
%     \toprule
%                     & explanation only & without explanation \\
%         \hline
%         \textbf{\movie}\\
%         \exptask &  \textbf{0.980} & 0.675\\
%         \mtlhard($\lambda=5.0$) & 0.960 & \textbf{0.487}\\
%         \human & 0.899 & 0.523\\
%         \hline\\
%         \textbf{\fever}\\
%         \exptask & 0.920 & \textbf{0.803}\\
%         \mtlhard($\lambda=20.0$) & 0.913 & 0.819\\
%         \human & \textbf{0.921} & 0.827\\
%         \hline\\
%         \textbf{\multirc}\\
%         \exptask & 0.761 & \textbf{0.623}\\
%         \mtlhard($\lambda=2.0$) & \textbf{0.745} & 0.630\\
%         \human & 0.759 & 0.633\\
%     \bottomrule
%     \end{tabular}
%     %}
%     \caption{The explanation quality of hard models}
%     \label{tab:hard_models_exp_quality}
% \end{table*}


\textcolor{red}{RQ4: \mtlsoft \ref{table:task_explanation_result_soft}}
\begin{table*}[tb]
    \centering
    \begin{tabular}{lcccc}
    \toprule
        & \textbf{Macro F1} & \textbf{AUPRC} & \textbf{Comprehensiveness$\uparrow$} & \textbf{Sufficiency$\downarrow$}\\
    \hline
    \textbf{\movie}\\
    BERT-LSTM + Attention & \textbf{0.974} & \textbf{0.467}  & 0.091 & \textbf{0.035}\\
    BERT-LSTM + Simple Gradient & \textbf{0.974} & 0.441 & 0.113 & 0.052\\
    \hline
    \mtlsoft($\lambda=50.0$) & 0.88 & 0.420 & \textbf{0.385} & 0.163\\
    \hline\\
    \textbf{\fever}\\
    GloVe-LSTM + Attention & 0.660 & 0.617 & -0.011 & 0.129\\
    GloVe-LSTM + Simple Gradient & 0.660 & 0.271 & 0.070 & 0.077\\
    \hline
    \mtlsoft($\lambda=5.0$) & \textbf{0.914} & \textbf{0.836} & \textbf{0.151} & \textbf{0.068}\\
    \hline\\
    \textbf{\multirc}\\
    BERT-LSTM + Attention & 0.655 & 0.240 & 0.145 & 0.085\\
    BERT-LSTM + Simple Gradient & 0.655 & 0.224 & \textbf{0.164} & 0.079\\
    \hline
    \mtlsoft($\lambda=2.0$) & \textbf{0.726} & \textbf{0.695} & 0.157 & \textbf{0.031}\\
    \bottomrule
    \end{tabular}
    \caption{Performance of \textbf{soft-selection} baseline models.}
    \label{table:task_explanation_result_soft}
\end{table*}



% In this section, we first evaluate the performance of the proposed MTL framework. Tables~\ref{table:task_explanation_result_hard} and~\ref{table:task_explanation_result_soft} report the performance of the baselines, \methodindv{}, and \methodspan{}. As mentioned earlier, baseline models are broadly of two categories (hard and soft selection) based on their rationale selection process. Table~\ref{table:task_explanation_result_hard} reports the result for hard rationale selection based baselines, \methodindv{}, and \methodspan. Performance of these baselines are measured in terms of \textbf{macro-avg-F1}, \textbf{IOU F1}, and \textbf{token F1} because such models contain rationale level supervision. On the other hand, results for soft-selection approaches are presented in Table~\ref{table:task_explanation_result_soft}. These models are trained only on task level data and do not have any explicit rationale level supervision. Hence, \textbf{Macro F1}, \textbf{AUPRC}, \textbf{Comprehensiveness}, and \textbf{Sufficiency} metrics are computed for these baselines.

% It is evident from Table~\ref{table:task_explanation_result_hard} that none of the methods perform consistently well across all the three metrics. However, \methodindv{} efficiently handles the trade-off between task prediction and rationale selection and keeps a consistent balance among all the three metrics. \methodindv{} shows better task performance (macro-avg-F1) for \fever{} and \multirc{} without significant drop in IOU F1 and token F1.

% Table~\ref{table:task_explanation_result_soft} highlights the effect of multi-task learning framework. \methodindv{} performs consistently well both in terms of task and rationale selection metrics. Higher value of  AUPRC  indicates that better choice of threshold of per token rationale prediction can help in improving explainability. Higher value of comprehensiveness indicates that \methodindv{} selects the correct rationales that are responsible for accurate task label prediction i.e., task performance drops significantly without these tokens. Low value of sufficiency also supports the fact i.e., it is an indication that model is able to learn the task well only based on those tokens. For \movie, BERT-LSTM + Attention is able to identify rationales well (low sufficiency) and high value of AUPRC indicates that rationales are in accordance with human annotated ones. However, the low value of comprehensiveness reveals that the model can still learn without those rationales that might lead to the option that attention based selections are not always rationales~\citet{jain2019attention}. On the other hand, \methodindv{} ensures that the rationales learned are in accordance with human rationales and the model performance significantly drops without those tokens. It fits with our objective that the models should be interpretable by design. However, \methodindv{} achieves high comprehensiveness but sufficiency is higher than the baselines. This suggests that our method is able to retrieve rationale tokens quite well but those are not sufficient to learn the task i.e., it fails to capture some rationale tokens. However, it is able to maintain a balance between task and rationale selection. 



% \textbf{What are the task-explanation performance trade-offs in an MTL framework?}



% \begin{table}[tb]
%     \centering
%     \resizebox{\linewidth}{!}{
%     % \begin{tabular}{lccc}
%     % \toprule
%     %           & \textbf{TASK} accuracy & \textbf{TASK Macro F1} & \textbf{EXP}-token-F1  \\
%     %     \hline
%     %      \textbf{\movie}&&\\
%     %      \textsc{TASK} & 0.894 & 0.894 & -\\
%     %      \textsc{Token} - EXP & - & - & 0.335 \\
%     %      %\textsc{Span} - EXP & - & - & 0.315 \\
%     %      \methodindv($\lambda=5.0$) & 0.879 & 0.869 & 0.324\\
%     %      %\methodspan($\lambda=0.1$) & 0.889 & & 0.140\\
%     %      \hline
%     %      \\
%     %      \textbf{\fever}\\ 
%     %      \textsc{TASK} & 0.917 & 0.916 & -\\
%     %      \textsc{Token} - EXP & - & - & 0.820 \\
%     %      %\textsc{Span} - EXP & - & - & 0.449 \\
%     %      \methodindv($\lambda=5.0$) & 0.914 & 0.914 & 0.831\\
%     %      %\methodspan($\lambda=0.2$) & 0.902 && 0.729\\
%     %      \hline
%     %      \\
%     %      \textbf{\multirc}&&\\
%     %      \textsc{TASK} & 0.721 & 0.708 & - \\
%     %      \textsc{Token} - EXP & - & - & 0.839 \\
%     %      %\textsc{Span} - EXP & - & - & 0.424 \\
%     %      \methodindv($\lambda=2.0$) & 0.730 & 0.726 & 0.599 \\
%     %      %\methodspan($\lambda=0.1$) & 0.692 & & 0.290\\
%     % \bottomrule
%     % \end{tabular}
%         \begin{tabular}{lcc}
%     \toprule
%               & \textbf{TASK Macro F1} & \textbf{EXP}-token-F1  \\
%         \hline
%          \textbf{\movie}&&\\
%          \textsc{TASK} & 0.894 & -\\
%          \textsc{Token} - EXP &  - & 0.335 \\
%          \methodindv($\lambda=5.0$) &  0.869 & 0.324\\
%          \hline
%          \\
%          \textbf{\fever}\\ 
%          \textsc{TASK} & 0.916 & -\\
%          \textsc{Token} - EXP & - & 0.820 \\
%          \methodindv($\lambda=5.0$) & 0.914 & 0.831\\
%          \hline
%          \\
%          \textbf{\multirc}&&\\
%          \textsc{TASK} & 0.708 & - \\
%          \textsc{Token} - EXP & - & 0.839 \\
%          \methodindv($\lambda=2.0$) & 0.726 & 0.599 \\
%     \bottomrule
%     \end{tabular}
%     \vspace{-3cm}
%     }
%     \caption{{\bf The individual \textsc{TASK} and EXPLANATION (EXP)  performance of MTL based models. \textbf{EXP}-token-F1 represents the token-wise rationale F1 for the sub-token inputs of \bert{}(sequence length $\leq512$). Metrics are taken from the ERASER~\citet{deyoung2019eraser}.}}
%     \label{table:mtl}
%     \vspace{-3mm}
% \end{table}

% In this part, our objective is to verify the effect of rationales on task performance and vice-versa. The motivation behind MTL is that there should not be any significant drop in task accuracy because of the explanation part i.e., it can effectively handle the task-explanation trade-off and both the task and explanation can take benefit from each other. Table~\ref{table:mtl} shows the effect of task and explanation based training scenarios. This trend is quite evident for \fever{} and \movie{}. In general, the explanation part works as a regularizer to improve the task prediction and avoid overfitting. A detailed analysis reveals that \methodspan{} has to learn a lot of parameters and performs worse than \methodindv{} due to overfitting issue. We leave the task of learning the impact of precise or general explanation structures on model performance as a future work.



% \noindent\textbf{What impact does $\lambda$ have on task and explanation performance?}

% \begin{figure}[tb] 
%   \centering 
%   \subfigure[\textbf{Classification Macro Average F1}]{ 
%     \label{fig:subfig:acc}
  
%     \includegraphics[width=0.48\columnwidth]{figs/task_f1.pdf}}

%   \subfigure[\textbf{Explanation Macro F1}]{ 
%     \label{fig:subfig:macro_f1}
%     \includegraphics[width=0.48\columnwidth]{figs/hard_exp_metric.pdf}}

%     \caption{Performance variation of task (a) and explanation (macro token/IOU-F1) (b) of \methodindv{} with $\lambda$ (log-scale) on the first 10\% \fever{} dataset. Here we can see the obvious contradiction between classification and explanation along the $\lambda$ increases}
    
%   \label{fig:lambda-sweep_1} 
% \end{figure}


% \begin{figure}[tb] 
%   \centering 

%   \subfigure[\textbf{Comprehensiveness and Sufficiency}]{ 
%     \label{fig:subfig:cs}
%     \includegraphics[width=0.48\columnwidth]{figs/comp_suff.pdf}}

%   \subfigure[\textbf{Explanation AUPRC}]{ 
%   \label{fig:subfig:auprc}
%     \includegraphics[width=0.48\columnwidth]{figs/auprc.pdf}}
%     \caption{{\bf Variation of comprehensiveness and sufficiency (a) and AUPRC of explanations (b) of \methodindv{} with $\lambda$ (log-scale) on the first 10\% \fever{} dataset.}}
    
%     \label{fig:lambda-sweep_2} 
% %   \vspace{-3mm}
% \end{figure}


% All the results reported so far are based on the $\lambda$ value that shows best performance on the validation set. In this part, we try to elaborate the effect of $\lambda$-sweep on both task and explanation. We observe an opposite trend in task and explanation i.e., the performance of the task decreases and explanation increases with the increased value of $\lambda$. In this part, we highlight the effect of $\lambda$-sweeping on the head 10\% \fever{} dataset\footnote{Similar trend is observed for other datasets.}. Figure~\ref{fig:lambda-sweep_1} (a) and (b) clearly reflect the contrasting effect. The task F1 score goes on decreasing while explanation scores (IOU F1, token F1) improve with increment of  $\lambda$. Task accuracy deteriorates rapidly after $\lambda\geq50$. Figure~\ref{fig:lambda-sweep_2}(d) supports the same trend i.e., rationale token AUPRC goes on increasing with $\lambda$. Slightly different trend is observed for comprehensiveness($\uparrow$) and sufficiency($\downarrow$). There is no monotonic increment and decrement in the performance with the variation in $\lambda$. Performance reaches a peak point within an interval and subsequently it starts to deteriorate. Hence, a careful selection $\lambda$ is required to effectively handle the trade-off between task and rationales.


% The values of $\lambda$'s in the table \ref{table:mtl} as well as \ref{table:downstream} are selected by increasing it in log-scale and select the one brings the best performance on the evaluation set. Intuitively, the greater $\lambda$ is, the more the final performance tilts to the explanation task, i.e. the performance of classification deteriorates and that of explanation improves. The figures in \ref{fig:lambda-sweep} verifies this hypothesis. These figures are based on results of $\lambda$-sweeping on the head 10\% of the \fever~dataset. The sub-figure \ref{fig:subfig:acc} indicates descending of classification accuracy along with increment of $\lambda$, while for the explanation metrics such as IOU-F1, Token-F1~\ref{fig:subfig:macro_f1} and AUPRC~\ref{fig:subfig:auprc} it is totally opposite. From the figure we can also tell that the accuracy rapidly deteriorates especially when $\lambda\geq50$, and the IOU- and Token-F1 keep on increasing tremendously before $\lambda\leq 1$. For the comprehensiveness (the higher the better) and sufficiency (the lower the better)~\ref{fig:subfig:cs} some other patterns emerge. It seems that for the comprehensiveness there is an optimal interval of $\lambda$, where it performs well, while the sufficiency decreases all the way through. Taking all those metrics into consideration, we need to find a $\lambda$ which induces high classification accuracy, high comprehensiveness, low sufficiency and high on F1-s and AUPRC, therefore $\lambda=5$ could be a good choice. The choosing of optimal $\lambda$-s for other structures and/or datasets follows analogy procedure. To save the page we leave other $\lambda$-sweeping figures to the appendix.



% \if 0
% \begin{figure*}[tb] 
%   \centering 
%   \subfigure[Classification Macro Average F1]{ 
%     \label{fig:subfig:acc}
%     \includegraphics[width=0.48\linewidth]{figs/lambda_sweep/fever_gru_val_train_on_portion_0_1_macro_avg_f1.png}}
%   \subfigure[Comprehensiveness and Sufficiency]{ 
%     \label{fig:subfig:cs}
%     \includegraphics[width=0.48\linewidth]{figs/lambda_sweep/fever_gru_val_train_on_portion_0_1_cs.png}}
%   \subfigure[Explanation Macro F1]{ 
%     \label{fig:subfig:macro_f1}
%     \includegraphics[width=0.48\linewidth]{figs/lambda_sweep/fever_gru_val_train_on_portion_0_1_iou_token_f1.png}}
%   \subfigure[Explanation AUPRC]{ 
%     \label{fig:subfig:auprc}
%     \includegraphics[width=0.48\linewidth]{figs/lambda_sweep/fever_gru_val_train_on_portion_0_1_auprc.png}}
%   \caption{Performance of \textit{cls} and \textit{exp} task in \methodindv w.r.t. 6 metrics on log-scale variation of $\lambda$ on the top 10\% data of~\fever. Horizontal lines and curves sharing same line type in each sub-figure correspond to the same metric, where the horizontal lines are the highest (for sufficiency the lowest) scores of each metrics out of all baseline models.}
%   \label{fig:lambda-sweep} 
% \end{figure*}
% \fi


% \begin{table*}
% \label{table:task_performance}
%     \centering
%     \begin{tabular}{l|c|c|c|c}
%              & \movie & \multirc & \fever~\\
%              \hline
%         \gru  - CLS&&&\\ 
%         \elmo - CLS&&&\\
%         \bert - CLS& 0.886 & 0.908 & 0.707 & 0.908\\
%         \bert - MTL & 0.XXX & 0.XXX & 0.XXX & 0.819\\
%     \end{tabular}
%     \caption{Task accuracy of three different models (task only)}
% \end{table*}
% Along side the classification, we need also to annotate explicit evidence supporting this classification on the input sentence. Conditions used in filtering objective twitters in \semsent{} (final.polarity\_in\_dataset!='neutral')
%               \& (final.subjectivity>0)
%               \& ((abs(final.polarity\_textblob) > 0.1))=>10196 out of 30466 instances passed this subjectivity test, where 6530 are used for testing, 699 for dev, 680 for devtest and 2061 fro training.


% \begin{table*}
% \label{table:task_performance}
%     \centering
%     \begin{tabular}{l|c|c|c|c}
%              & \imdb & \semsent & \semirony & \zaidan \\
%              \hline
%         \gru  - EXP &&&\\ 
%         \elmo - EXP &&&\\
%         \bert - EXP & 0.XXX & 0.XXX & 0.XXX & 0.941\\
%         \bert - MTL & 0.XXX & 0.XXX & 0.XXX & 0.931\\
%     \end{tabular}
%     \caption{Explanation Accuracy of three different models}
% \end{table*}

% bert with length of sequence == 128
%------------------------
% bert@ACL IMDB:
% {'auc': 0.88628,
%  'eval_accuracy': 0.88628,
%  'f1_score': 0.8865658,
%  'false_negatives': 1390.0,
%  'false_positives': 1453.0,
%  'global_step': 2343,
%  'loss': 0.4798463,
%  'precision': 0.8843429,
%  'recall': 0.8888,
%  'true_negatives': 11047.0,
%  'true_positives': 11110.0}
%-----------------------------
%bert @ imdb length == 512
% {'auc': 0.93851995,
%  'eval_accuracy': 0.93852,
%  'f1_score': 0.9382606,
%  'false_negatives': 821.0,
%  'false_positives': 716.0,
%  'loss': 0.35001868,
%  'precision': 0.94223475,
%  'recall': 0.93432,
%  'true_negatives': 11784.0,
%  'true_positives': 11679.0,
%  'global_step': 9375}
 %---------------------------
 % bert@semeval 2016 sentiment seq_len=128
%  {'auc': 0.87515986,
%  'eval_accuracy': 0.90816325,
%  'f1_score': 0.93506485,
%  'false_negatives': 255.0,
%  'false_positives': 690.0,
%  'global_step': 494,
%  'loss': 0.37832594,
%  'precision': 0.9079263,
%  'recall': 0.9638759,
%  'true_negatives': 2541.0,
%  'true_positives': 6804.0}
%bert@semeval2016 sentiment seq_len=512
% {'auc': 0.8695189,
%  'eval_accuracy': 0.90767735,
%  'f1_score': 0.93525964,
%  'false_negatives': 197.0,
%  'false_positives': 753.0,
%  'loss': 0.4629555,
%  'precision': 0.9011162,
%  'recall': 0.9720924,
%  'true_negatives': 2478.0,
%  'true_positives': 6862.0,
%  'global_step': 1978}
%-----------------------------
% bert@semeval 2018 irony seq_len=128
% {'auc': 0.70947224,
%  'eval_accuracy': 0.70790815,
%  'f1_score': 0.6607407,
%  'false_negatives': 88.0,
%  'false_positives': 141.0,
%  'global_step': 357,
%  'loss': 0.8956044,
%  'precision': 0.61263734,
%  'recall': 0.7170418,
%  'true_negatives': 332.0,
%  'true_positives': 223.0}
%---------------------
%bert@semeval 2018 irony seq_len=512
% {'auc': 0.7169602,
%  'eval_accuracy': 0.71428573,
%  'f1_score': 0.66961646,
%  'false_negatives': 84.0,
%  'false_positives': 140.0,
%  'loss': 1.2306125,
%  'precision': 0.6185286,
%  'recall': 0.7299035,
%  'true_negatives': 333.0,
%  'true_positives': 227.0,
%  'global_step': 1431}
% ---------------------------------
% bert@zaidan07
% {'auc': 0.9079837,
%  'eval_accuracy': 0.90833336,
%  'f1_score': 0.9115281,
%  'false_negatives': 13.0,
%  'false_positives': 20.0,
%  'global_step': 135,
%  'loss': 0.18267174,
%  'precision': 0.8947368,
%  'recall': 0.92896175,
%  'true_negatives': 157.0,
%  'true_positives': 170.0}
%--------------------------------------
%--------------------------------------
%bert with max_seq_length=512
% {'auc': 0.99397594,
%  'eval_accuracy': 0.99444443,
%  'f1_score': 0.99487174,
%  'false_negatives': 0.0,
%  'false_positives': 2.0,
%  'loss': 0.027238758,
%  'precision': 0.9897959,
%  'recall': 1.0,
%  'true_negatives': 164.0,
%  'true_positives': 194.0,
%  'global_step': 540}.0}
%---------------------------------------
%---------------------------------------
%gru on zaidan07 with max_seq_length=128, batch_size=64, learning_rate=1e-2,epoch=15,num_gru_units=128, embedding_size=100
% {'auc': 0.81780726,
%  'eval_accuracy': 0.82222223,
%  'f1_score': 0.7974683,
%  'false_negatives': 43.0,
%  'false_positives': 21.0,
%  'loss': 0.4920561,
%  'precision': 0.85714287,
%  'recall': 0.74556214,
%  'true_negatives': 170.0,
%  'true_positives': 126.0,
%  'global_step': 42}
%-----------------------------
%gru on imdb 
% {'auc': 0.77712005,
%  'eval_accuracy': 0.77712,
%  'f1_score': 0.76419795,
%  'false_negatives': 3471.0,
%  'false_positives': 2101.0,
%  'global_step': 732,
%  'loss': 0.5287146,
%  'precision': 0.8112309,
%  'recall': 0.72232,
%  'true_negatives': 10399.0,
%  'true_positives': 9029.0}
%-----------------------------------------
%gru on SemEval16(sent)
% {'auc': 0.5,
%  'eval_accuracy': 0.68600583,
%  'f1_score': 0.81376445,
%  'false_negatives': 0.0,
%  'false_positives': 3231.0,
%  'loss': 0.6292327,
%  'precision': 0.68600583,
%  'recall': 1.0,
%  'true_negatives': 0.0,
%  'true_positives': 7059.0,
%  'global_step': 154}
%------------------------------
%gru on SemEval18(sarcasm)max_seq_len=64
% {'auc': 0.6604046,
%  'eval_accuracy': 0.6619898,
%  'f1_score': 0.605067,
%  'false_negatives': 108.0,
%  'false_positives': 157.0,
%  'loss': 0.6578578,
%  'precision': 0.5638889,
%  'recall': 0.65273315,
%  'true_negatives': 316.0,
%  'true_positives': 203.0,
%  'global_step': 745}
%----------------------------------------
%----------------------------------------
%bert on ration(seq) zaidan07
%val_acc: 0.9411


==> trash bin/acknowledgments.tex <==
\section*{Acknowledgments}

The acknowledgments should go immediately before the references. Do not number the acknowledgments section.
Do not include this section when submitting your paper for review.
